Budgeted Out-tree Maximization with Submodular Prizes

We consider a variant of the prize collecting Steiner tree problem in which we are given a \emph{directed graph} $D=(V,A)$, a monotone submodular prize function $p:2^V \rightarrow \mathbb{R}^+ \cup \{0\}$, a cost function $c:V \rightarrow \mathbb{Z}^{+}$, a root vertex $r \in V$, and a budget $B$. The aim is to find an out-subtree $T$ of $D$ rooted at $r$ that costs at most $B$ and maximizes the prize function. We call this problem \emph{Directed Rooted Submodular Tree} (\textbf{DRSO}). Very recently, Ghuge and Nagarajan [SODA\ 2020] gave an optimal quasi-polynomial-time $O\left(\frac{\log n'}{\log \log n'}\right)$-approximation algorithm, where $n'$ is the number of vertices in an optimal solution, for the case in which the costs are associated to the edges. In this paper, we give a polynomial-time algorithm for \textbf{DRSO} that guarantees an approximation factor of $O(\sqrt{B}/\epsilon^3)$ at the cost of a budget violation of a factor $1+\epsilon$, for any $\epsilon \in (0,1]$. The same result holds for the edge-cost case, to the best of our knowledge this is the first polynomial-time approximation algorithm for this case. We further show that the unrooted version of \textbf{DRSO} can be approximated to a factor of $O(\sqrt{B})$ without budget violation, which is an improvement over the factor $O(\Delta \sqrt{B})$ given in~[Kuo et al.\ IEEE/ACM\ Trans.\ Netw.\ 2015] for the undirected and unrooted case, where $\Delta$ is the maximum degree of the graph. Finally, we provide some new/improved approximation bounds for several related problems, including the additive-prize version of \textbf{DRSO}, the maximum budgeted connected set cover problem, and the budgeted sensor cover problem.

==> Extra-Material.tex <==
\iffalse
Then it constructs an edge-cost graph $D''=(V'', A'')$ of $D'$ such that $V''=V'$, $A''=A'$ and for any $e=(i, j) \in A''$, $c'(e)=c(j)$ (Line~\ref{lnEdgeCost}). Then, for any vertex $u \in V''$, it finds all the vertices $ V_u \subseteq V''$ such that for any $v \in V_u$, $dist(u, v) \le \lfloor \sqrt{B} \rfloor$ (Line~\ref{lnEdgeCost}). By applying Lemma~\ref{lmKuoMRS}, for any vertex $u \in V'$, Algorithm~\ref{algNW-DRBP} finds a set $Sol_u$ with cost at most $c(u)+\lfloor \sqrt{B} \rfloor$ nodes from set $V_u$ which one is $u$, i.e., $u \in Sol_u$ (Line~\ref{lnMRS}). Nodes in $Sol_u$ are not necessary reachable from $u$ in the directed graph induced by set $Sol_u$ but the distance from $u$ to any $v \in Sol_u$ is at most $\lfloor \sqrt{B} \rfloor$ on $D''$. It iteratively repeats this process for any vertex $u \in V''$ and picks the one for which $p(Sol_u)$ is maximized, i.e., $u^*=argmax_{u \in V''} p(Sol_u)$. Note that as for any $v \in V$, $c(v) \in \mathbb{Z}^+$, then the number of nodes in $Sol$ is at most $\lfloor \sqrt{B} \rfloor +1$. In order to have any $v \in Sol\setminus \{u^*\}$ reachable from $u^*$, %, we are allowed to have at most $B-\lfloor \sqrt{B} \rfloor$ extra nodes, respecting the budget constraint, as $|Sol| \le \lfloor \sqrt{B} \rfloor$. To do so, for any vertex $v \in Sol_{u^*}$, 
Algorithm~\ref{algNW-DRBP} adds all the edges along a shortest path from $u^*$ to $v$ to a tree $T$, i.e., $T=\{P(u^*, v)| v \in Sol_{u^*}\setminus \{u^*\}\}$, where $P(u^*, v)$ is a shortest path from $u^*$ to $v$ (Line~\ref{lnAddingShortestPathBegin}-\ref{lnAddingShortestPathEnd}). Since $|Sol_{u^*} \setminus \{u^*\}| \le \lfloor \sqrt{B} \rfloor$ and the distance from $u^*$ to any vertex $v \in V_{u^*}$ is at most $ dist(u^*, v) \le \lfloor \sqrt{B}\rfloor$, then the total cost of tree $T$ is at most $c(u^*)+\lfloor \sqrt{B} \rfloor \times \lfloor \sqrt{B} \rfloor \le c(u^*)+B$. %extra nodes we add is at most $(\lfloor \sqrt{B} \rfloor-1) \times (\lfloor \sqrt{B} \rfloor-1) \le B-\lfloor \sqrt{B} \rfloor$. 
In the next step, Algorithm~\ref{algNW-DRBP} checks whether $r^*=u^*$. If it is the case, we are done and $c(T)\le 2B$ (assuming that $c(r^*) \le B$). Otherwise, to have $r^*$ as the root of $T$, Algorithm~\ref{algNW-DRBP} adds a shortest path $P$ from $r^*$ to $u^*$, i.e., $T=T \cup P$, then it removes all the entering edges of vertices of $P$ on $T$ (Line~\ref{lnAdding-r-toSolutionBgin}-\ref{lnAdding-r-toSolutionEnd}). This edge-removing process ensures that the final solution $T$ will be a tree. As $D'$ is a $B$-appropriate graph of $D$ for $r^*$, the cost from $r^*$ to $u^*$ is no more than $B$, implying that adding this path to the final solution may cost us an extra budget $B$, which means that $c(T) \le 2B$. Let $\gamma=\frac{p(T)}{c(T)}$. Last, Algorithm~\ref{algNW-DRBP} applies Corollary~\ref{coTrimmingProcess} to $T$ and obtain a new arborescence $T$ with prize-to-cost ratio $\frac{\epsilon \gamma}{4}$ (Line~\ref{lnTrimmingProcess}). 
\fi



%Next we aim to extend Lemma~\ref{lmClaimKuoExtension} to a more general case. We call a directed graph $D'=(V', A')$ connected if any vertex $v \in V'$ is reachable from at least one vertex $u \in V'$, i.e., there exists a path from some vertex $u$ to any vertex $v \in V$. 
%Consider the unrooted version of \textbf{NW-DRBP}, where the goal is to find an out-arborescence $T$ rooted at an arbitrary vertex $u$, such that $c(T) \le B$ and $p(T)$ is maximized. We term this variant of \textbf{NW-DRBP}, \textbf{NW-DBP}. Note that in \textbf{NW-DBP} no distinguished vertex is specified to be the root of $T$. 

%\begin{corollary}\label{coCorollaryKuoExtension}
%There always exist $N \le 6 \lfloor \sqrt{B} \rfloor$ of directed connected subgraphs $D^i=(V^i, A^i)$ of graph $D_{OPT_B}$, where $D_{OPT_B}$ is the directed connected subgraph of $D$ induced by $OPT_B$, $A^i=V^i \times V^i \cap A$, $c(V^i) \le c(u_i)+\sqrt{B}$ %and any vertex $v \in V^i$ is reachable from $u_i$ in the graph induced by $V^i$ for all $1 \le i \le N$ such that $\bigcup_{i=1}^{N} V^i =OPT_B$.
%\end{corollary}

%\begin{proof}
%Keep in mind that any vertex $v \in OPT_B$ is reachable from at least one vertex $r$ in $D_{OPT_B}$. Let $T_{OPT_B}$ be an arbitrary out-arborescence $D_{OPT_B}$ rooted at $r$. By substituting $T_{OPT_B}$ and $\lfloor \sqrt{B} \rfloor$ for $T$ and $m$ used in Lemma~\ref{lmClaimKuoExtension}, respectively, there exist at most $N \le 6 \lfloor \frac{B}{\sqrt{B}} \rfloor= 6 \lfloor \sqrt{B} \rfloor$ out-subarborescences $T^i=(V^i, A^i)$ of $T_{OPT_B}$, where $c(V^i) \le \sqrt{B}+c(r_i)$ and $r_i$ is the root of $T^i$, for all $1 \le i \le N$ such that $\bigcup_{i=1}^{N} V_i=OPT_B$. This finishes the proof.%This implies that there always exist at most $N+1=N' \le 6 \lfloor \sqrt{B} \rfloor$ directed connected subgraphs $D^i=(V^i, A^i)$ of graph $D_{OPT_B}$. directed connected subgraphs $D^i=(V^i, A^i)$ of graph $D_{OPT_B}$ such that $c(V^i) \le c(u_i)+\sqrt{B}$ and any vertex $v \in V^i$ is reachable from $u_i$ in the graph induced by $V^i$ for all $1 \le i \le N'$ such that $\bigcup_i^{N'} V^i =OPT_B$.
%\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%$$Apply the trimming process in Lemma~\ref{lmBateniTrimmingProcessGeneral} to $T$ and return $T$.  


%Let $OPTR_{B}$ be an optimal solution to \textbf{NW-DRBP} when the budget is $B$. Recall that $OPT_{B}$ is an optimal solution to \textbf{NW-DBP} when the budget is equal to $B$. The general idea of proof is that we first claim that Algorithm~\ref{algNW-DRBP} provides a solution $T_z$ with $ p(OPT_B)=O(\sqrt{B}) p(T_z)$ to \textbf{NW-DBP} (this claim will be proved later in this proof). Now as $OPTR_{B}$ is a feasible solution to \textbf{NW-DBP}, $p(OPT_B) \ge p(OPTR_{B})$. Now if $z=r$, i.e., $T=T_z$, we are done and $c(T) \le 2B$. Otherwise, we compute a solution by adding to $T_{z}$ a shortest path $P$ from $r$ to $z$ and removing the edges in $E(T_{z})\setminus E(P)$ incoming the nodes in $V(T_{z})\cap V(P)$. Let $T$ be our solution with prize $p(T) = O(\frac{1}{\sqrt{B}}) p(OPT_{B})$ and cost $c(T) \le 2B$ (because each vertex on $D$ has a distance no more than $B$ from $r$). This implies that Algorithm~\ref{algNW-DRBP} finds an arborescence with prize-to-cost ratio $\gamma=\frac{OPT_{B}}{O(\sqrt{B})2B}$. By Lemma~\ref{lmBateniTrimmingProcessGeneral}, it will find another arborescence $T$ rooted at $r$ of the cost $\epsilon B/2 \le c(T) \le (1+\epsilon)B$ and the prize-to-cost ratio:

%\[
%\frac{p(T)}{c(T)} \ge \frac{\epsilon^2 \gamma}{32} \ge \frac{\epsilon^2 p(T)}{32 B} = O(\frac{\epsilon^2}{\sqrt{B}B}) OPT_{B}.
%\]

%As $c(T) \ge \epsilon B/2$, we have $p(T) = O( \frac{\epsilon^3}{\sqrt{B}}) OPT_{B}$. %As an optimal solution $OPT_{RB}$ to \textbf{NW-DRBP} is a feasible solution to \textbf{EW-DBP}, then we have $O(\sqrt{B})p(Sol) \ge p(OPT_B) \ge p(OPT_{RB})$. Note that in case $u^* \ne r^*$, we only need to add a directed shortest path from $r^*$ to $u^*$ and pay an extra cost at most $B$.


%It remains to show that $ p(OPT_B)=O(\sqrt{B})p(T)$. Let $OPT'$ be the optimal solution to an instance $I^{BSM}_u$ of the knapsack problem with elements $V_u$, budget $\sqrt{B}$, where $V_u$ is the set of vertices having distance at most $\lfloor \sqrt{B} \rfloor$ from $u$. Let $u$ be an vertex in $OPT_{c(u)+\lfloor \sqrt{B}\rfloor}$ such that any vertex in $OPT_{c(u)+\lfloor \sqrt{B}\rfloor}$ is reachable from $u$. Hence, $OPT_{c(u)+\lfloor \sqrt{B}\rfloor} \subseteq V_u$. So, $OPT_{c(u)+\lfloor \sqrt{B}\rfloor}$ is a feasible solution to $I^{BSM}_u$ and thus $p(OPT') \ge p(OPT_{c(u)+\lfloor \sqrt{B}\rfloor})$. Then, by Lemma~\ref{lmKuoMRS}, we have $\frac{e}{e-1} p(Sol_u) \ge OPT' \ge p(OPT_{c(u)+\lfloor \sqrt{B}\rfloor})$. As Algorithm~\ref{algNW-DRBP} selects a vertex $u^*$ such that $p(Sol_{u^*})$ is maximized, where $Sol_{u^*} \subseteq Sol$. Then, 

%$$\frac{e-1}{e}p(Sol) \ge \frac{e-1}{e}p(Sol_{u^*}) \ge \frac{e-1}{e}p(Sol_u) \ge \frac{e-1}{e}p(OPT_{c(u)+\lfloor \sqrt{B}\rfloor}).$$

%Therefore, by Lemma~\ref{lmLemmaKuoExtension}, we have

%$$\frac{e-1}{e}O(\sqrt{B}p(Sol)) \ge \frac{e-1}{e}O(\sqrt{B} p(OPT_{c(u)+\lfloor \sqrt{B}\rfloor})) \ge p(OPT_B).$$
 
%This concludes the proof.

==> RelatedWork/RelatedWork.tex <==
\section{Related Work}\label{secRW}

\textit{Prize collecting problems} are very well-known problems and many variants of these problems have been investigated. Here we list the prize collecting problems related to our study.

\paragraph{Submodular Tree Orienteering (\textbf{STO}).} Ghuge and Nagarajan~\cite{ghuge2020quasi} introduced this problem, which is as follows. Given directed graph $D=(V, A)$, a vertex $r^* \in V$, a budget $B$, a monotone submodular function $f: 2^V \rightarrow \mathbb{R}^+$ and a cost $c:A \rightarrow \mathbb{Z}^+$, and the goal is to find out-directed arborescence $T^*=(V(T^*), A(T^*))$, rooted at $r^*$ and maximizes $ f(V(T^*))$ such that $ \sum_{e\in A(T^*)}c(v) \le B$. 

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{STO}\\
		\emph{Input}: a directed graph $ D= (V, A)$, a monotone submodular $f: 2^V \rightarrow \mathbb{R}^+$, a cost function $c: A \rightarrow \mathbb{Z}^+$, a specific vertex $r^* \in V$ and a budget $B\in\mathbb{N}$.\\
		\emph{Feasible Solution}: an out-directed arborescence $T=(V(T), A(T))$ rooted at $r^*$ s.t. $c(T)=\sum_{e \in A(T)} c(e)\le B$. \\
		\emph{Goal}: $f(V(T))$ maximized.
}}\\
\end{center}

Ghuge and Nagarajan~\cite{ghuge2020quasi} provided a quasi-polynomial time $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for \textbf{STO} that runs in
$(n \log B)^{O(\log^{1+\epsilon} n')}$ time for any constant $\epsilon > 0$, where $n'$ is the number of vertices in an optimal solution. The authors mentioned that this factor is tight for \textbf{STO} in quasi-polynomial time. Ghuge and Nagarajan~\cite{ghuge2020quasi} pointed out that their technique provides a quasi-polynomial time $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for \textbf{DTO} (Directed Tree Orienteering), which is the special case of \textbf{STO} in which the accumulated prize of out-directed arborescence $T=(V(T), A(T))$ is obtained by a linear function, i.e., $f(T)=\sum_{v \in V(T)} p(v)$ and $p:V \rightarrow \mathbb{Z}^+$. D'Angelo, Delfaraz and Gilbert~\cite{dangelo2022computation} studied a special case of \textbf{DTO} in Liquid Democracy systems, where the costs on edges are either $0$ or $1$. The authors provided a polynomial-time bicriteria $(1+\epsilon, \frac{8n}{\epsilon^2 B})$-approximation algorithm and some parametrized complexity results for this problem. The authors pointed out that their technique provides a polynomial-time bicriteria $(1+\epsilon, \frac{8B'}{\epsilon^2 B} )$-approximation algorithm for \textbf{DTO}, where $B'$ is the cost of the minimum spanning tree rooted at $r^*$.

%\paragraph{Directed Tree Orienteering \textbf{DTO}.} Ghuge and Nagarajan~\cite{ghuge2020quasi} introduced this problem, which is the same as \textbf{STO} and the only difference is that the monotone submodular function $f$ is replaced by an additive prize function $p:V \rightarrow \mathbb{Z}^+$.

%\begin{center}
%\noindent\fbox{\parbox{14cm}{
%		\emph{Problem}: \textbf{DTO}\\
%		\emph{Input}: a directed graph $ D= (V, A)$, a prize function $p: V \rightarrow \mathbb{R}^+$, a cost function $c: A \rightarrow \mathbb{Z}^+$, a specific vertex $r^* \in V$ and a budget $B\in\mathbb{N}$.\\
%		\emph{Feasible Solution}: an out-directed arborescence $T=(V(T), A(T))$ rooted at $r^*$ s.t. $c(T)=\sum_{e \in A(T)} c(e)\le B$. \\
%		\emph{Goal}: $p(T)=\sum_{v \in V(T)} p(v)$ maximized.
%}}\\
%\end{center}

%Ghuge and Nagarajan~\cite{ghuge2020quasi} pointed that their quasi-polynomial time $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for \textbf{STO} can be directly applied to \textbf{DTO}. The authors mentioned that this factor is tight for \textbf{DTO} in quasi-polynomial time. 


\paragraph{Directed Steiner Tree Problem (\textbf{DSTP}).} This is a very well-known problem:

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{DSTP}\\
		\emph{Input}: a directed graph $ D= (V, A)$, a cost function $c: A \rightarrow \mathbb{Z}^+$, a specific vertex $r^* \in V$ and a subset $U \subseteq V$ of terminals.\\
		\emph{Feasible Solution}: an out-directed arborescence $T=(V(T), A(T))$ rooted at $r^*$ s.t. $U \subseteq V(T)$. \\
		\emph{Goal}: $c(T)=\sum_{e \in A(T)} c(e)$ minimized.
}}\\
\end{center}

Zelikovsky~\cite{zelikovsky1997series} provided the first approximation algorithm for \textbf{DSTP} with factor $O(k^{\epsilon} (\log^{1/\epsilon}{k}))$ that runs in $O(n^{1/\epsilon})$, where $|U|=k$. Charikar et al.~\cite{charikar1999approximation} proposed a better approximation algorithm for \textbf{DSTP} with a factor $O(\log^3{k})$ in quasi-polynomial time. Grandoni et al.~\cite{grandoni2019log2} improved this factor and provided a randomized $O(\frac{\log^2 k}{\log \log k})$-approximation algorithm $n^{O(\log^{5} k)}$ time. Also, they showed that, unless $NP \subseteq \bigcap_{0 <\epsilon< 1} \text{ZPTIME}(2^{n^\epsilon})$ or the Projection Game Conjecture is false, there is no quasi-polynomial time algorithm for \textbf{DSTP} that achieves an approximation ratio of $o(\frac{\log^2 k}{\log \log k})$. Ghuge and Nagarajan~\cite{ghuge2020quasi} showed that their quasi-polynomial time approximation algorithm for \textbf{DTO} results in a deterministic $O(\frac{\log^2 k}{\log \log k})$-approximation algorithm for \textbf{DSTP} in $n^{O(\log^{1+\epsilon} k)}$ time. 


\paragraph{Maximum Connected Submodular function with Budget constraint (\textbf{MCSB}).}
Kuo et al.~\cite{kuo2014maximizing} considered the following problem. %Given a connected graph $G=(V, E)$ with a cost function $c:V \rightarrow \mathbb{Z}^+$, a nondecreasing submodular function $f$ on the set of subset of $V$ with $f(\emptyset)=0$ and a positive integer $B$. The MCSB problem asks for a subset $S\subseteq V$ such that: 1) $S$ is a connected with respect to $G$; 2) the weight of $S$ is no larger than $B$, i.e., $c(S)=\sum_{v \in S}c(v) \le B$; 3) $f(S)$ is maximized.

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{MCSB}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a monotone submodular function $f: 2^V \rightarrow \mathbb{R}^+$, a cost function $c: V \rightarrow \mathbb{Z}^+$ and a budget $B$.\\
		\emph{Feasible Solution}: A connected set $S$ s.t.  $c(S)=\sum_{v \in S}c(v) \le B$. \\
		\emph{Goal}: $f(S)$ is maximized.
}}\\
\end{center}


Kuo et al.~\cite{kuo2014maximizing} provided a $O(\Delta \sqrt{B})$-approximation algorithm for \textbf{MCSB}, where $\Delta$ is the maximum degree. One of the main application of \textbf{MCSB} is in wireless sensor networks, where the goal is to find a connected set of sensors to maximize the number of covered users using no more than $B$ sensors. We term this problem Budgeted Sensor Cover Problem (\textbf{BSCP}). Kuo et al.~\cite{kuo2014maximizing} pointed out that their technique implies a $\frac{5(\sqrt{B}+1)}{1-1/e}$-approximation algorithm for \textbf{BSCP}. Very recently, Xu et al.~\cite{xu2021throughput} improved this result and gave a $\frac{\lfloor\sqrt{B}\rfloor}{1-e}$-approximation algorithm for \textbf{BSCP}. Gao et al.~\cite{gao2018algorithm} provided two approximation algorithms with factors $O(\log{n})$ and $O(\sqrt{B})$ for this problem. Huang, Jian and Qicai~\cite{huang2020approximation} proposed a $\frac{8(\lceil 2\sqrt{2} C\rceil+1)^2}{1-1/e}$-approximation algorithm for \textbf{BSCP}, where $C=\frac{R_s}{R_c}$, $R_c\le R_s$, $R_s$ and $R_c$ are the sensing range and communication range of sensors, respectively. Danilchenko et al.~\cite{danilchenko2020covering} investigated a closely related problem in which there are a set $S$ of $n$ points distributed in the plane, each point $s_i$ is assigned with a positive prize $p(s_i)$ and a set $P$ of $m$ disks (or squares) of radius $R$, and the goal is to place them such that the covered points by $P$ have the maximum prize and set $P$ should be connected. Danilchenko et al.~\cite{danilchenko2020covering} provided a polynomial-time $O(1)$-approximation algorithm for this problem.



\textbf{MCSB} is also closely related to budgeted connected dominating set problem, where the goal is to select at most $B$ connected vertices in a given undirected graph to maximize the profit function on the set of selected vertices. Khuller, Purohit and Sarpatwar~\cite{khuller2020analyzing} investigated this problem in which the profit function is a \textit{special submodular function} $f$, where $f$ is submodular and $f(A \cup X)-f(A)=f(A\cup B \cup X)-f(A\cup B)$ if $N(X)\cap N(B)=\emptyset$ $\forall X,A,B \subseteq V$, where $N(X)$ is the neighborhood of $X$ including itself. Khuller, Purohit and Sarpatwar~\cite{khuller2020analyzing} designed a $\frac{12}{1-1/e}$-approximation algorithm. By generalizing the analysis of Khuller, Purohit and Sarpatwar~\cite{khuller2020analyzing}, Lamprou, Sigalas and Zissimopoulos~\cite{lamprou2020improved} showed that there is a $\frac{11}{1-e^{-7/8}}$-approximation algorithm for the budgeted connected dominating set problem. They also showed that $1-1/e$-approximation guarantee is tight for this problem unless $P=NP$. Vandin, Upfal and Raphael investigated a special case of \textbf{MCSB}, which was motivated by the discovery of mutated driver pathways in cancer. They provided a $(\frac{2e-1}{e-1}r)$-approximation algorithm, where $r$ is the radius of optimal solution in the given graph $G$. This problem coincides with the connected maximum coverage problem in which each set has cost one. In the connected maximum coverage problem, we are given a set $X$ of elements, a collection sets $\mathcal{S} \subseteq 2^X$, a prize function $p: X \rightarrow \mathbb{R}^+$, a cost function $c: \mathcal{S} \rightarrow \mathcal{R}^+$, a graph $G$ on vertex set $\mathcal{S}$, and a budget $B$. The goal here is to find a subcollection $\mathcal{S}'\subseteq \mathcal{S}$ such that $c(\mathcal{S}')=\sum_{S \in \mathcal{S}'}c(S) \le B$, the subgraph induced by $\mathcal{S}'$ is connected and $p(\mathcal{S}')=\sum_{x \in X_{\mathcal{S}'}} p(x)$ is maximized, where $X_{\mathcal{S}'}=\bigcup_{S \in \mathcal{S}'} S$. Ran et al.~\cite{ran2016approximation} investigated this problem under the assumption that two sets $S$ and $S'$ having an element in common are adjacent, and provided a $((\Delta+1)\log{n})$-approximation algorithm. Hochbaum and Rao~\cite{hochbaum2020approximation} investigated \textbf{MCSB}, where each vertex costs $1$ for the detection of mutated driver pathways in cancer and provided an approximation algorithm with factor $\min\{\frac{1}{(1-1/e)(1/R-1/B)}, B\}$, where $R$ is the radius of the
input graph $G$. As \textbf{STO} is a more general case of \textbf{MCSB}, the technique by Ghuge and Nagarajan~\cite{ghuge2020quasi} provides a quasi-polynomial time $O(\frac{\log n'}{\log \log n'})$-approximation algorithm for all of the above problems.% and their directed versions.


\paragraph{Node-Weighted Rooted Budgeted Problem (\textbf{NW-RBP}).}

In this problem we are looking for a tree including a distinguished vertex $r$ such that the tree has the maximum weight, while its cost respects the given budget constraint. More formally,

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{NW-RBP}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: V \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$ and a budget $B$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$ and $c(T)=\sum_{v \in V(T)}c(v) \le B$. \\
		\emph{Goal}: $p(T)=\sum_{v\in V(T)} p(v)$ is maximized.
}}\\
\end{center}

Guha et al.~\cite{guha1999efficient} introduced this problem and proposed a polynomial time $(\log^2 {n})$-approximation algorithm for \textbf{NW-RBP} that violates the budget constraint by a factor of $2$. Moss and Rabbani~\cite{moss2007approximation} showed that one can use an $\alpha$-approximation algorithm for \textbf{NW-PCST} as a black-box method and provide a bicriteria $(2, O(\alpha))$-approximation algorithm for \textbf{NW-RBP}, that is, there is an $O(\alpha)$-approximation algorithm for \textbf{NW-RBP} which exceeds the budget constraint by a factor of at most $2$. Thus, using the ideas of K{\"o}nemann, Sadeghian and Sanita~\cite{konemann2013lmp}, Bateni, Hajiaghayi and Liaghat~\cite{bateni2018improved}, one can provide a bicriteria $O(1+\epsilon, \frac{\log(n)}{\epsilon^2})$-approximation algorithm for \textbf{NW-RBP}. Also, the trimming process proposed by Bateni, Hajiaghayi and Liaghat~\cite{bateni2018improved} enables us to have an $O(\log{n})$-approximation algorithm for the unrooted version of \textbf{NW-RBP} without violating the budget limit. Recall that Kortsarz and Nutov~\cite{kortsarz2009approximating} showed that the unrooted version of \textbf{NW-RBP}, so does \textbf{NW-RBP}, admits no bicriteria $(\rho, o(\log \log n))$-approximation algorithm, where $\rho$ is a universal constant, unless $NP \subseteq DTIME(n ^{\text{polylog}(n)})$.

%   have the \textit{rooted budgeted problem} in which we are given an undirected graph $G=(V, E)$, a vertex $r \in V$, a budget $B$, each vertex $v$ is associated with a prize $\pi(v)$ and a cost $c(v)$, and the goal is to find a subtree $T=(V(T), E(T))$ of $G$, such that $c(T)=\sum_{v \in V(T)}c(v) \le B$ and $\pi(T)=\sum_{v\in T(V)}\pi(v)$ is maximized. As mentioned by K{\"o}nemann, Sadeghian and Sanita, using their idea and the separation oracle presented by Moss and Rabbani~\cite{moss2007approximation} lead us to an $O(\log n)$-approximation algorithm for the rooted budgeted problem which exceeds the budget by a factor of $2$. Bateni, Hajiaghayi and Liaghat~\cite{bateni2018improved} proposed a new trimming process and used the main idea of Moss and Rabbani~\cite{moss2007approximation} to provide a bicriteria $O(1+\epsilon, \frac{\log(n)}{\epsilon^2})$-approximation algorithm for the rooted budgeted problem, where $\epsilon > 0$.

\paragraph{Edge-Weighted Rooted Budgeted Problem (\textbf{EW-RBP}).}

This is the same as \textbf{NW-RBP}, while the costs are on the edges. More formally,

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{EW-RBP}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: E \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$ and a budget $B$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$ and $c(T)=\sum_{e \in E(T)}c(e) \le B$. \\
		\emph{Goal}: $p(T)=\sum_{v\in V(T)} p(v)$ is maximized.
}}\\
\end{center}

Johnson, Minkoff and Phillips~\cite{johnson2000prize} introduced \textbf{EW-RBP} and showed that there exists a $5+\epsilon$-approximation algorithm for the unrooted version of \textbf{EW-RBP} using Garg's $3$-approximation algorithm~\cite{garg3} for the $k$-MST problem. Later this approximation ratio is improved to $4+\epsilon$ by Levin~\cite{levin2004better}. Johnson, Minkoff and Phillips~\cite{johnson2000prize} also observed that a $2$-approximation algorithm for $k$-MST would yield a $3$-approximation algorithm for the unrooted version of \textbf{EW-RBP}. So, Garg's $2$-approximation algorithm~\cite{garg2005saving} for $k$-MST gives us such a guarantee. Recently, Paul et al.~\cite{paul2020budgeted} provided a polynomial-time $2$-approximation algorithm for \textbf{EW-RBP} and its unrooted version. Zhou et al.~\cite{zhou2018relay} studied a variant of \textbf{EW-RBP} in the wireless sensor networks, called the Relay Node Placement Problem (\textbf{RNPP}). In \textbf{RNPP}, we are given the location of a set $P=\{p_1, p_2, \dots, p_n\}$ of sensor nodes (terminal points) in the Euclidean plane, the communication range $R$ of sensor nodes and a budget $B$ on the relay nodes can be placed in the deployment area. The aim in \textbf{RNPP} is to find a set $Q$ with $|Q| \le B$ points in the plane where the relay nodes can be deployed such that the largest connected component in the graph induced by set $P \cup Q$ is maximized. Zhou et al.~\cite{zhou2018relay} provided a $10$-approximation algorithm for \textbf{RNPP}. Seufert et al.~\cite{seufert2010bonsai} investigated a special case of the unrooted version of \textbf{NW-RBP}, where each vertex has cost $1$ and we aim to find a tree with at most $B$ nodes maximizing the accumulated prize. This coincides with the unrooted version of \textbf{EW-RBP} when the cost of each edge is $1$ and we are looking for a tree containing at most $B-1$ edges to maximize the accumulated prize. Seufert et al.~\cite{seufert2010bonsai} provided a $(5+\epsilon)$-approximation algorithm for this problem. Similarly, Huang et al.~\cite{huang2019maximizing} investigated this variant of \textbf{EW-RBP} (or \textbf{NW-RBP}) in plane. In particular, we are given a set $\mathcal{D}$ of $n$ unit disks in the plane and an integer $k$, and the goal is to find a subset $\mathcal{D}' \subseteq \mathcal{D}$ with $|\mathcal{D}'| \le k$ such that the covered area by $\mathcal{D}'$ is maximized and the unit disks in $\mathcal{D}'$ are connected. Huang et al.~\cite{huang2019maximizing} proposed a $2$-approximation algorithm for this problem.


\paragraph{Node-Weighted Rooted Quota Problem (\textbf{NW-RQP}).}

Here we wish to find a tree including a vertex $r$ in a way that the total cost of the tree is minimized and its prize is more than some \textit{quota}.

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{NW-RQP}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: V \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$ and a quota $Q$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$ and $p(T)=\sum_{v \in V(T)} p(v) \ge Q$. \\
		\emph{Goal}: $c(T)=\sum_{v\in V(T)} c(v)$ is minimized.
}}\\
\end{center}


Moss and Rabbani~\cite{moss2007approximation} showed that we can also use an $\alpha$-approximation algorithm for \textbf{NW-PCST} as a black-box method and provide a $(2 \alpha+1)$-approximation algorithm for \textbf{NW-RQP} where the output tree has a prize more than or equal to $Q$. So, with the ideas of K{\"o}nemann, Sadeghian and Sanita~\cite{konemann2013lmp}, and Bateni, Hajiaghayi and Liaghat~\cite{bateni2018improved}, we have an $O(\log{n})$-approximation algorithm for \textbf{NW-RQB}. This bound is tight~\cite{moss2007approximation}.

\paragraph{Edge-Weighted Rooted Quota Problem (\textbf{EW-RQP}).} Here we have the edge weighted version of \textbf{EW-RQB}.

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{EW-RQP}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: E \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$ and a quota $Q$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$ and $ p(T)=\sum_{v \in V(T)} p(v) \ge Q$. \\
		\emph{Goal}: $c(T)=\sum_{e\in E(T)} c(e)$ is minimized.
}}\\
\end{center}


Johnson, Minkoff and Phillips~\cite{johnson2000prize} investigated \textbf{EW-RQP} and showed that by adapting an $\alpha$-approximation algorithm for the $k$-MST problem (in which we wish to find a tree with the minimum cost that spans at least $k$ vertices), one can have an $\alpha$-approximation algorithm for \textbf{EW-RQP}. Hence, the $2$-approximation algorithm of Garg~\cite{garg2005saving} for the $k$-MST problem results in a $2$-approximation algorithm for \textbf{EW-RQP}.

\paragraph{Node-Weighted Prize-Collecting Steiner Tree (\textbf{NW-PCST}).} Given an undirected graph $G=(V, E)$, a vertex $r \in V$, each vertex $v$ is associated with a prize (or penalty) $p(v)$ and a cost $c(v)$, and the goal is to find a subtree $T=(V(T), E(T))$ of $G$, such that $r \in V(T)$ and $\sum_{v \in V(T)}c(v)+ \sum_{v\in V\setminus V(T)} p(v)$ is minimized. 

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{NW-PCST}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: V \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$. \\
		\emph{Goal}: $\sum_{v \in V(T)}c(v)+ \sum_{v\in V\setminus V(T)}p(v)$ is minimized.
}}\\
\end{center}

Moss and Rabani~\cite{moss2007approximation} studied this problem and some of its variants. K{\"o}nemann, Sadeghian and Sanita~\cite{konemann2013lmp} provided a Lagrangian multiplier preserving $O(\ln{n})$-approximation algorithm for \textbf{NW-PCST}. Bateni, Hajiaghayi and Liaghat~\cite{bateni2018improved} considered a more general case of \textbf{NW-PCST} and that their approach results is an $O(\log{n})$-approximation algorithm for \textbf{NW-PCST}. There exists no $o(\ln{n})$-approximation algorithm for \textbf{NW-PCST}, unless $NP \subseteq \text{DTIME}(n^{\text{Polylog}(n)})$~\cite{klein1993nearly}.

\paragraph{Edge-Weighted Prize-Collecting Steiner Tree (\textbf{EW-PCST}).} This is an edge weighted variant of \textbf{NW-PCST}, which is as follows

\begin{center}
\noindent\fbox{\parbox{14cm}{
		\emph{Problem}: \textbf{EW-PCST}\\
		\emph{Input}: An undirected graph $G=(V, E)$, a prize function $p: V \rightarrow \mathbb{Z}^+$, a cost function $c: E \rightarrow \mathbb{Z}^+$, a specific vertex $r \in V$.\\
		\emph{Feasible Solution}: A subtree $T=(V(T), E(T))$ s.t. $ r \in V(T)$. \\
		\emph{Goal}: $\sum_{e \in E(T)}c(e)+ \sum_{v\in V\setminus V(T)} p(v)$ is minimized.
}}\\
\end{center}

Goemans and Williamson~\cite{goemans1995general} provided a $2$-approximation algorithm for \textbf{EW-PCST}. Archer et al.~\cite{archer2011improved} proposed a $(2-\epsilon)$-approximation algorithm for \textbf{EW-PCST} which was an improvement upon the long standing bound of $2$.


\begin{table}[ht!]
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 Problem & Best Bound \\ \hline
 \textbf{STO} & $O(\frac{\log{n}}{\log{\log{n}}})$~\cite{ghuge2020quasi} (tight) \\ \hline
 \textbf{DTO} & $O(\frac{\log{n}}{\log{\log{n}}})$~\cite{ghuge2020quasi} (tight) \\ \hline
 \textbf{DSTP} & $O(\frac{\log^2{k}}{\log{\log{k}}})$~\cite{ghuge2020quasi, grandoni2019log2} (tight) \\ \hline
 \textbf{NW-PCST} & $O(\log{n})$~\cite{bateni2018improved, konemann2013lmp} (tight) \\ \hline
  \textbf{EW-PCST} & $2-\epsilon$~\cite{archer2011improved} \\ \hline
 \textbf{NW-RBP} & $(1+\epsilon, O(\frac{\log{n}}{\epsilon^2}))$~\cite{bateni2018improved, konemann2013lmp, moss2007approximation} \\ \hline
 \textbf{EW-RBP} & $2$~\cite{paul2020budgeted} \\ \hline
 \textbf{NW-RQP} & $O(\log{n})$~\cite{bateni2018improved, konemann2013lmp, moss2007approximation} (tight)\\ \hline
 \textbf{EW-RQP} & $2$~\cite{garg2005saving, johnson2000prize} \\ \hline
\end{tabular}
\caption{A summary of the best bounds on some variants of prize collecting problems.}\label{tbBestBounds}
\end{center}
\end{table}

\HG{Very good table, Thank you.}

==> contribution/Application/Budgeted-Connected-Dominating-Set.tex <==
\paragraph{Budgeted Connected Dominating Set (\textbf{BCDS}).} 




==> contribution/Application/STO.tex <==
\paragraph{Submodular Tree Orienteering (\textbf{STO}).} Ghuge and Nagarajan~\cite{ghuge2020quasi} introduced this problem, whuch is the same problem as \textbf{NW-DRBP} except that edges and not nodes have costs. Here we provide the first polynomial-time approximation algorithm for \textbf{STO}.

%a more general case of \textbf{NW-DRBP}, called \textbf{STO}. In \textbf{STO}, we have the same input as \textbf{NW-DRBP} except the prize function is a monotone submodular function $f: 2^V \rightarrow \mathbb{R}_+$ and an edge cost function $c:A \rightarrow \mathbb{R}_+$ and the goal is to find out-arborescence $T$ rooted at $r^*$ of cost at most $B$ that maximizes $f(T)$.

\begin{theorem}\label{thDTOAlgorithm1}
There exists a polynomial-time bicriteria $(1+\epsilon, O(\frac{\sqrt{B}}{\epsilon^3}))$-approximation algorithm for \textbf{STO}.
\end{theorem}

\begin{proof}[Sketch of proof]
We first transform the given instance $I$ of \textbf{STO} to an instance $J$ of \textbf{NW-DRBP} as Lemma~\ref{thGhugeEW-RDBPQuasiAlgorithm}. Now we can run Algorithm~\ref{algNW-DRBP} on $J$ with some minor changes. As the cost of each edge in $I$ is at least $1$, in Line 4 of the algorithm we can select at least $1$ one vertex and most $\sqrt{B}$ vertices. By a binary search and the greedy algorithm of Nemhauser et al.~\cite{nemhauser1978analysis}, we can find a set of vertices $I^{BSM}_z$ with maximum prize that costs at most $\sqrt{B}$. The rest of algorithm is the same. In a manner analogous to that
of Theorem~\ref{thMain}, the theorem is concluded.
\end{proof}

%To the best of our knowledge, this is the first polynomial-time approximation algorithm for \textbf{STO}.
\paragraph{Node Weighted Rooted Budget (\textbf{NW-DRB})}.

\textbf{NW-DRB} is the special case of \textbf{NW-DRBP} where the prize function $p$ is an additive function, i.e., $p: V\rightarrow \mathbb{R}^+ \cup \{0\}$ and for any $S \subseteq V$, $p(S)=\sum_{v \in S} p(v)$. We apply algorithm~\ref{algNW-DRBP} to \textbf{NW-DRB} but we have two changes: (i) in Line 4 of the algorithm, we instead define an instance $I^{Knap}_u$ of the Knapsack problem with elements $V_u$, budget $\sqrt{B}$, profit $p(I^{Knap}_u)=\sum_{v \in I^{Knap}_u} p(v)$ and cost $c(v)$, for each $v\in V_u$ and apply an $1-\epsilon$-approximation algorithm to $I^{Knap}_u$ in Line 5 and, (ii) in Line 12 of the algorithm, we instead use a different trimming process to achieve a better approximation factor. To do this, we show that Lemma~\ref{lmBateniTrimmingProcess} can be applied to directed graphs and results in the same guarantee.

Let us first briefly explain the trimming process by Bateni et al.~\cite{bateni2018improved}. We are given an undirected graph $G=(V, E)$, a distinguished vertex $r \in V$ and a budget $B$, where each vertex $v \in V$ is assigned with a prize $p'(v)$ and a cost $c'(v)$. Let $T$ be a tree, where $V(T) \subseteq V$ and $E(T) \subseteq E$ and let  $c'(T)=\sum_{v \in V(T)} c'(v)$ and $p'(T)=\sum_{v \in V(T)} p'(v)$. The trimming procedure by Bateni et al. takes  as input an out-subtree $T$ rooted at a node $r$ of a $B$-proper graph $G$ and first (i) computes an out-subtree $T''$ of $T$, not necessarily rooted $r$, such that $\frac{\epsilon B}{2}\leq c'(T'') \leq \eps B$ and $p'(T'')\geq \frac{\eps B}{2}\gamma$, where $\gamma = \frac{p'(T)}{c'(T)}$. Then (ii) connects node $r$ to the root of $T''$ with a minimum-cost path and obtain a tree $T'$ rooted at $r$. Since $G$ is $B$-proper, this path exists and has length at most $B$, which implies that the cost of the resulting tree is between $\frac{\epsilon B}{2}$ and $(1+\eps)B$, and its prize to cost ratio is at least $\frac{p'(T'')}{(1+\eps)B}\geq\frac{\epsilon \gamma}{4}$. This leads to Lemma~\ref{lmBateniTrimmingProcess}. For directed graph we prove a lemma equivalent to Lemma~\ref{lmBateniTrimmingProcess}.

\begin{lemma}\label{coTrimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $T$ be an out-arborescence of $D$ rooted at $r$ with prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}$. Suppose that for $\epsilon \in (0, 1]$, $c(T) \ge \frac{\epsilon B}{2}$. One can find an out-arborescence $T'$ rooted at $r$ with prize-to-cost ratio at least $\frac{\epsilon \gamma}{4}$ such that $\epsilon B/2 \le c'(T') \le (1+\epsilon)B$.
\end{lemma}
\begin{proof}
\iffalse
The trimming process used by Bateni et al. computes a subtree $T''$ of the original tree $T$ with $c'(T'') \leq \eps B$ and $p'(T'')\geq \frac{\eps B}{2}\gamma$ and then connects node $r$ to the root of $T''$ in order obtain $T'$. Since the underlying graph is $B$-proper, this path exists and has length at most $B$, which implies that the cost of the resulting tree is at most $(1+\eps)B$ and the prize to cost ratio is at least $\frac{p(T'')}{(1+\eps)B}\geq\frac{\epsilon \gamma}{4}$. 
\fi
We first define an undirected tree by removing the directions from $T$ and apply to it the step (i) of the trimming procedure by Bateni et al. with $p'(\cdot) = p(\cdot)$ and $c'(\cdot) =c(\cdot)$ as prize and cost functions, respectively. We obtain a subtree $T''$ such that $\frac{\epsilon B}{2}\leq c'(T'') \leq \eps B$ and $p'(T'')\geq \frac{\eps B}{2}\gamma$. We reintroduce in $T''$ the same directions as in $T$  to obtain an out-arborescence $T''_{out}$ corresponding to $T''$. Then, we add a minimum cost path from $r$ to the root of $T''_{out}$. Since $D$ is $B$-appropriate, this path exists and has length at most $B$. The obtained out-arborescence $T'$ has the desired properties because $p(T''_{out}) = p'(T'') $ and $ c(T''_{out}) = c'(T'')$ and therefore $\frac{\epsilon B}{2}\leq c(T')\leq (1+\eps)B$ and $\frac{p(T')}{c(T')}\geq\frac{p'(T'')}{(1+\eps)B}\geq\frac{\epsilon \gamma}{4}$.
\end{proof}

This results in the following theorem.

\begin{theorem}\label{thNWDRBAlgorithm1}
There exists a polynomial-time bicriteria $(1+\epsilon, O(\frac{\sqrt{B}}{\epsilon^2}))$-approximation algorithm for \textbf{NW-DRB}.
\end{theorem}
\begin{proof}[Sketch of proof]
By using the same argument as that of Theorem~\ref{thMain} and Lemma~\ref{coTrimmingProcess}, the theorem is concluded.
\end{proof}




\paragraph{ Directed Tree Orienteering (\textbf{DTO}).} 

This is the same problem as \textbf{STO} instead the prize function is an additive function. By using Theorems~\ref{thSTOAlgorithm1} and~\ref{thNWDRBAlgorithm1}, we have the following.

\begin{theorem}\label{thSTOAlgorithm1}
There exists a polynomial-time bicriteria $(1+\epsilon, O(\frac{\sqrt{B}}{\epsilon^2}))$-approximation algorithm for \textbf{DTO}.
\end{theorem}




==> contribution/In-Degree-One.tex <==
\subsection{\textbf{NW-DRBP} on Graphs with In-Degree at most 1}
There is a pseudo-polynomial time algorithm for \textbf{NW-DRBP} when in a given graph $D=(V, A)$ for any vertex $v \in V$, $|\mathtt{Nb}_{in}(v)| \le 1$.


\begin{theorem}\label{thNW-DRBPPseudo-Polynomial}
There is a pseudo-polynomial time algorithm for \textbf{NW-DRBP} whose running time is $O(n^2p_{max})$ on directed graphs $D=(V, A)$ where $p_{max}=\max_{v \in V} p(v)$ such that for any vertex $v \in V$, $|\mathtt{Nb}_{in}(v)| \le 1$.
\end{theorem}

\begin{proof}
By removing the incoming-edge of $r^*$  if there is one, the vertices reachable from $r^*$ are on an out-tree, say $T=(V_T, A_T)$, rooted at $r^*$. Now we proceed as follows. If $\sum_{e \in A_T} c(e) \le B$, we are done \HG{Can't the weights be negative no?}. Suppose it is not the case. Then we proceed as follows. Let $V_T=\{1,2,\dots, n\}$ be the set of vertices in $T$ and $n=r^*$. We run a depth-first search of $T$ starting from $r^*$. Let $\pi_d$ be the ordering of vertices in $T$ such that vertices are sorted in decreasing order of their discovering times in the depth first search. 
As $n$ is first visited in the depth first search, it is the last voter in the ordering $\pi_d$. We define a table $F$ where $F[i,p]$ is the subtree with composed of a set $S \subseteq \{1,2,\dots, i\}$ with prize exactly $p$ and whose cost is minimized, where $i$ ranges from $0$ to $n-1$ and $p$ ranges from $1$ to $np_{max}$ \HG{Once again the weights can be negative, why $n-1$ and not $n$ ?}. Let $T(j) \subseteq T$ be the subtree rooted in a vertex $j$ and $t_j=|T(j)|$. Note that a subtree rooted at a vertex $j$ consists of all vertices whose path to the root of $T$ passes through $j$. The entries of this table will be filled as follows. For $i=0$ and $p \in \{1, \dots, np_{max}\}$ we have $F[0,p]=0$. For any $i$ and $p < p(i)$, we have $F[i,p]=F[i-t_i,p]$. When $p(i) \le p$, we define $F[i,p]=\min \{F[i-1, p-p(i)]+c_i, F[i-t_i, p]\}$. The first summand corresponds to the case that $i$ will be in the solution and there will be a path from $r^*$ to $i$. The second summand indicates that $i$ will not be in the solution, so $i$ and of course the subtree $T(i)$ will be removed from further consideration. After filling the table entries, we can determine which entry of the table contains the optimal weight to \textbf{EW-RBP} whose cost is less than or equal to $B$ as follows: $OPT=\max\{p| F[n-1, p] \le B\}$. Now comparing the first summand and the second summand will enable us to find out whether $i$ (and possibly its subtree) is in the final solution. Thus it takes $O(n^2p_{max})$ time to find an optimal solution.
\end{proof}

We can utilize the FPTAS given for the Knapsack problem to present an FPTAS for \textbf{NW-DRBP} on trees. 
\begin{theorem}
    There exists an FPTAS for \textbf{NW-DRBP} on trees that runs in $O(n^2 \left \lfloor{\frac{n}{\epsilon}}\right \rfloor )$, where $n$ is the number of vertices and $\epsilon >0$.
\end{theorem}

\begin{proof}
Let $T$ be the given tree. Let $P_T(i,j)$ be the path from vertex $i$ to $j$ in $T$ and $c(P_T(i,j))=\sum_{e \in P_T(i,j)} c(e)$. Let $V_{reach} $ be the set of vertices $v$ in $T$ such that $c(P_T(r^*,v)) \le B$. Given $\epsilon >0$ and let $K=\frac{\epsilon p_{max}}{n}$, where $p_{max}=max_{v \in V_{reach}} p(v)$ \HG{Rephrase sentence}. We can set a new prize for each vertex $v \in V$ as $p'(v)=\left \lfloor{\frac{p(v)}{K}}\right \rfloor$. Now we can run the given dynamic-programming algorithm in Theorem~\ref{thNW-DRBPPseudo-Polynomial} for new weights. Let $T'$ be an optimal solution for \textbf{NW-DRBP} on the new instance (i.e., the instance obtained from updating prizes). Let $T^*$ be an optimal tree before updating the prizes. Because of rounding down, $K.p'(v) \le p(v)$ for any $v \in V(T)$ \HG{Why ?}. So, we have 

$$p(T^*)-K.p'(T^*) \le nK.$$

The dynamic-programming algorithm must return a set at least as good as $T^*$ under the new prizes. Let $OPT=p(T^*)$. Therefore,

\begin{align*}
    p(T') \ge K.p'(T^*) \ge p(T^*)-nK=OPT- \epsilon p_{max} \ge (1-\epsilon) OPT,
\end{align*}
where the last inequality holds as $OPT \ge p_{max}$ \HG{This may not be true if weights can be negative but this can be solved}.
\end{proof}


==> contribution/Parametrized-Complexity.tex <==
\subsection{Parametrized Complexity of \textbf{NW-DRBP}}
We next show that \textbf{NW-DRBP} is NP-hard even when the out-degree and in-degree of every vertex in an SN is at most $2$, the weight assigned to each vertex is either $0$ or $1$ and the cost assigned to each edge is either $0$ or $1$. \ED{The idea here is as the one we presented for WMaxP.}


%\textbf{EW-DRBP} cannot be approximated with an approximation ratio better than $2$, assuming the unique games conjecture, even when all vertices have weight at most one.
\begin{comment}

\begin{theorem}\label{thIn-Degree-Out-Degree-At-Most2}
\textbf{NW-DRBP} cannot be approximated with an approximation ratio better than $O(1/(\ln n))$ even when in a given graph $D=(V,A)$, for any voter $i \in V$, $|\mathtt{Nb}_{out}(i)| \le 2$, \ $|\mathtt{Nb}_{in}(i)| \le 2$ and $\omega(i) \in \{0, 1\}$, and for any edge $e \in A$, $c(e) \in \{0,1\}$.
\end{theorem}

\begin{proof}
To prove the theorem, we give a reduction from the decision version of minimum vertex cover problem, called DMVC to the decision version of \textbf{NW-DRBP}, called \textbf{DDTO}. In DMVC, we are given a universe $ U = \{x_1,\ldots, x_N\}$ of $N$ elements, a collection $ P=\{ S_1, S_2, ..., S_m \} $ of $m$ subsets of $U$, and an integer $k$. The goal is to pick at most $k$ sets $S_{i_1},\ldots,S_{i_k}$ such that $|\bigcup_{j=1}^{k} S_{i_j}|=N$, i.e., $U$ is covered by $\bigcup_{j=1}^{k} S_{i_j}$. This problem cannot be approximated better than within a factor of $(1 - o(1)) \ln N$ unless $P = NP$~\cite{dinur2014analytical}. Note that in \textbf{DDTO}, we need to find a subtree $T^*$ of cost at most $B$ and weight at least $\tau$, where $\tau  \in \mathbb{Z}^+$.

Given an instance $I=(U, P, k)$ of DMVC, an instance $I=\langle D= (V, A), c, \omega, r^*, B, \tau \rangle$ of \textbf{DDTO} obtained as follows. We create a digraph $D = (V, A)$ where:

\begin{itemize}
    \item{For each element $x \in U$, we create a voter $v_{x}$ with weight $\omega(v_x)=1$. These voters will be called element vertices in the following.} 
    
    \item {A vertex $r^*$ is created.}
    
    \item{For each set $S \in P$, we create two vertices $v_S$ and $v'_S$ with weight $\omega(v_S)=\omega(v'_S)=0$. $v_S$ will be called a set vertex in the following. Then, an edge $e=(v'_S, v_S)$ of cost $1$ is created. Let $A'$ denote the set of such edges.}
    
    \item {For every $x \in U$ and $S \in P$, where $x \in S$, one vertex $v_{Sx}$ of weight $\omega(v_{Sx})=0$ is created. Then, we create an edge $e=(v_{Sx}, v_x)$ with cost $c(e)=0$}.
    
    \item {For every set $S=\{x_1, \dots, x_{|S|}\}$, we create edges $e=(v_{Sx_{i}}, v_{Sx_{i-1}})$ of cost $c(e)=0$, where $i \in [2, \dots, |S|]$. Also, an edge $e=(v_S, v_{Sx_{|S|}})$ of cost $0$ is created.}
    
    \item For the collection of sets $P=\{S_1, \dots, S_m\}$, we create edges $e=(v'_{S_{i}}, v'_{S_{i-1}})$ of cost $c(e)=0$, where $i \in [2, \dots, m]$. Last an edge $e=(r^*, v_{S_m})$ of cost $0$ is created.
    \item We define a budget $B=k$ and $\tau=N$.
  \end{itemize}		 
     
     
First we show that instance $I$ has a solution of size at most $k$ if and only if $D=(V, A)$ includes a subtree $T'$ with weight $\tau=N$ and cost at most $B=k$. Assume that there are a collection $SP$ of sets $S_{i_1},\ldots,S_{i_k}$ that cover all elements in $I$. Let $V_{SP}=\{v_{S_{i_1}}, \dots, v_{S_{i_k}}\}$ be the corresponding vertex sets collection $SP$ in $V$. Since $SP$ covers all elements, there exists at least one path from vertex sets in $V_{SP}$ to any element vertex $v_x \in V$ (the choice can be made arbitrary if several sets cover $x$ in $SP$). Note that any edge $e \in A' \subset A$, costs $1$ and $e \in A\setminus A'$ costs $0$. This concludes the first direction as the total cost is $B=k$. For the other direction, let $T'$ be a solution to \textbf{DUTO} such that $\omega(T')=N$ and $c(T') \le k$. As vertex elements are the only vertices with weight $1$, $T'$ must include all vertex elements. This implies that there exists a vertex sets $V'$ of size at most $k$, as $B=k$, such that from a vertex $v_S \in V'$ there exists a path to an element vertex $v_x \in V$. Thus the corresponding sets $V'$ in $P$ are a set cover in $I$.

Now let $k$ be the optimal value of the minimum set cover and $SP_{k}=\{v_{S_{i_1}}, \dots, v_{S_{i_k}}\}$ be an optimal solution. Let $\mathcal{A}$ be an algorithm for the minimum cover problem with approximation ratio $c \ge 1$. Now after running the algorithm $\mathcal{A}$ on instance $I$, the number of elements that is covered is equal to $N$ and the number of sets that is selected is at most $c.k$, denoted by $V_{EP}=\{v_{S'_{i_1}}, \dots, v_{S'_{i_{ck}}}\}$. Let $\mathcal{A'}$ be an algorithm that, given the graph $D=(V, A)$ resulting from our reduction, runs $\mathcal{A}$ to find a vertex sets that covers all element vertices. As $\mathcal{A'}$ outputs a tree $T'$ with cost at most $c.k$, we need to obtain a tree $T^*$ obtained from $T'$ that consists of $k$ vertex sets $V_{SP}=\{v_{S'_{i_1}}, \dots, v_{S'_{i_k}}\}$ out of $c.k$ vertex sets in $V_{EP}$ to respect the budget as $B=k$. %Without loss of generality assume that each vertex set in $V_{EP}$ covers almost the same number of vertex elements (and possibly vertex sets $V_{EP}$ have no vertex elements in common). 
As $ck$ vertex sets can cover all vertex elements, then $k$ vertex sets can cover at least $O(\frac{N}{c})$ vertex elements in the worst case, assuming $NP \ne P$. Hence, $\omega(T^*) \ge O(\frac{N}{c})$, which concludes the proof.
\end{proof}
\end{comment}


Consider the decision version of \textbf{NW-DRBP}, called \textbf{DNW-DRBP}, where the goal is to find a subtree $T$ rooted in $r^*$ with weight at least $\tau$, i.e, $\omega(T) \ge \tau$. Now we want to show that \textbf{DNW-DRBP} is $W[1]$-hard with respect to budget $B$. We provide a reduction from a specific version of the vertex cover problem to \textbf{DNW-DRBP}.

\begin{theorem}\label{thVertexCover-DT}
\textbf{DNW-DRBP} is $W[1]$-hard with respect to budget $B$.
\end{theorem}

\begin{proof}
To prove the theorem, we give a reduction from the following version of vertex cover problem, called Maximum Partial Vertex Cover (MPVC). Given a graph $G=(V, E)$ and two integers $k$ and $l$, the task in MPVC is to find a vertex set $V' \subset V$ with $|V'| \le k$ that covers at least $l$ edges. Guo, Niedermeier and Wernicke~\cite{guo2005parameterized} showed that MPVC is $W[1]$-hard with respect to $k$.

Now we construct an instance $I=\langle D= (\bar V, A), p, c, r^*, c, B, \tau \rangle$ of \textbf{DNW-DRBP} from an instance $I'=\langle G= (V, E), k, l \rangle$ of MPVC as follows. We create a digraph $D = (\bar V, A)$ where: 
\begin{itemize}
    \item $\bar V = V_1 \cup V_2 \cup \{r^*\} $ with $V_1 = \{w_e : e \in E\}$ and $V_2=\{u_i: i\in V\}$.
    \item $ A = \{(u_i, w_e) \in V_2 \times V_1 : i \in e \} \cup \{(r^*, u_i): i \in V\}$.
\end{itemize}

For any vertex $ w_e \in V_1 \subset A$, we set $c(w_e)=0$, for any $u_i \in V_2$, $c(u_i)=1$ and $c(r^*)=p(r^*)=0$. For any $w_e \in V_1$ and $u_i \in V_2$, let $p(w_e)=1$ and $p(u_i)=0$, respectively. We set $\tau=l$ and $B=k$. It is straight forward to see that $G$ has a vertex cover of size $k$ covering at least $l$ edges if and only if $D$ has an out-arborescence $T^*$ rooted at $r^*$ with weight $p(T^*) \ge l$.
\end{proof}


Following the idea of Ganian et al.~\cite{ganian2014digraph}, we can show that \textbf{NW-DRBP} remains $NP-hard$ even on graph classes that are restricted very beyond having small \textit{DAG-width}, $K$-\textit{width} and \textit{DAG-depth}. The reader can refer to Ganian et al.~\cite{ganian2014digraph} for definitions of $K$-width and DAG-depth. 

\begin{theorem}
\textbf{NW-DRBP} is NP-hard on DAGs (Directed Acyclic Graphs) of DAG-width $1$, $K$-width $2$ and DAG-depth $3$.
\end{theorem}

\begin{proof}
We give the same reduction as Theorem~\ref{thVertexCover-DT} from the vertex cover problem to \textbf{NW-DRBP}. The resulting graph $D$ obtained from the reduction is a DAG, so it has DAG-width $1$ as it is acyclic and $D$ itself will suffice as a decomposition. Following Ganian et al.~\cite{ganian2014digraph}, $D$ has $K$-width $2$ and DAG-depth $3$.
%, since there are only two paths from $r^*$ to each $w_e \in V_1$, only one path from $r^*$ to each $u_i \in V_2$ and only one path from each $v \in V_2$ to $w_e \in V_1$.
\end{proof}

More positively, \textbf{NW-DRBP} becomes tractable with respect to clique-width when the cost of each node is $1$. In particular, following Courcelle et. al~\cite{courcelle2000linear} and Ganian et al.~\cite{ganian2014digraph}, $LinEMSO_1$ optimization problems are defined as follows. Consider any \textit{MSO}$_1$ (monadic second order) formula $\Psi(X_1, \dots, X_p)$ with free set variables, and state the following problem on an input (di)graph $G=(V, E)$:

\begin{align*}
    opt\{f_{lin}(W_1, \dots, W_p): W_1, \dots, W_p \subseteq V, G \models \Psi(W_1, . . . , W_p)\},
\end{align*}
where $opt$ can be min or max, and $f_{lin}$ is a linear evaluation function. It is 

\begin{align*}
    f_{lin}(W_1, \dots, W_p)=\sum_{i=1}^{p} \sum_{j=1}^{m}(a_{i,j}.\sum{x \in W_i} f_j(x))
\end{align*}

where $m$ and $a_{i,j}$ are (integer) constants and $f_j$ are (integer) weight functions on the vertices of $G$. Then we have the following.

\begin{theorem}[Result of Ganian et al.~\cite{ganian2014digraph}]\label{thGanian-Cliqu-Width}
For every integer $t$ and $MSO_1$ formula $\Psi$, every $\Psi$-LinEMSO$_1$ optimization problem is fixed parameter tractable on digraphs of clique-width $t$, with the parameters $t$ and $|\Psi|$.
\end{theorem}

Also,  by following Gurski, Wanke and Yilmaz~\cite{gurski2016directed}, we have a more general result than Theorem~\ref{thGanian-Cliqu-Width}.


\begin{theorem}[Gurski, Wanke and Yilmaz~\cite{gurski2016directed}]\label{thGurski}
Every problem expressible in MSO$_1$-logic is fixed parameter tractable with respect to the parameters bi-rank-width, directed clique-width, and directed NLC-width.
\end{theorem}


Now we show that \textbf{NW-DRBP} belongs to the $\Psi$-LinEMSO$_1$ optimization problems when the cost of each node is $1$, so is tractable when parametrized by clique-width.

\begin{theorem}\label{thCliqueWidth2}
\textbf{NW-DRBP} is fixed parameter tractable when parametrized by bi-rank-width, directed clique-width, and directed NLC-width, where the cost of each node is $1$.
\end{theorem}

\begin{proof}
Given a digraph $D=(V, A)$. We reformulate \textbf{NW-DRBP} as to maximize the weight of $ r^* \in X \subseteq V$ such that $X$ induces in $D$ directed path from $r$ to all vertices of $X$. We can thus write

$$\sigma(r^*, X)\equiv r^* \in X \land (|X| \le B) \land \forall Z \subseteq X(r^* \in Z \rightarrow \exists x \in Z, y \in X \setminus Z.arc(x,y))$$

where $B$ is the budget. In particular, this formula says that we wish to find a set of vertices $X$ with size at most $B$ such that for any subset $Z \subseteq X$, $r^* \in Z$ and there exists at least one arc $(x, y)$ between $Z$ and $X\setminus Z$, where $x \in Z$ and $y \in X\setminus Z$. Then, the goal is 

$$max \{\sum_{x \in X} p(x): X \subseteq V, D \models \sigma(r^*, X)\}$$.

By Theorems~\ref{thGanian-Cliqu-Width} and~\ref{thGurski}, the proof is complete.
\end{proof}






==> contribution/Quasi-Polynomial-Time-Algorithm.tex <==
\subsection{A Quasi-Polynomial Time Algorithm}
In this section, we show that there is a quasi-polynomial time $O(\frac{\log k}{\log \log k})$-approximation algorithm for \textbf{NW-DRBP}, where $k \le n=|V|$ is the number of vertices in an optimal solution. Before proving this, we need some observations. First note that Ghuge and Nagarajan~\cite{ghuge2020quasi} investigated \textbf{STO} and showed that 

\begin{theorem}[Theorem 1 from Ghuge and Nagarajan~\cite{ghuge2020quasi}]\label{thGhugeEW-RDBPQuasiAlgorithm}
There is an $O(\frac{\log k}{\log \log k})$-approximation
algorithm for \textbf{DTO} that runs in
$(n \log B)^{O(\log^{1+\epsilon} k)}$ time for any constant $\epsilon > 0$, where $k \le n=|V|$ is the number of vertices in an optimal solution.
\end{theorem}

Now we prove that \textbf{NW-DRBP} and \textbf{STO} are equivalent from the approximability point of view.


\begin{lemma}\label{lmApproximabilityDTOandNW-DRBP}
Consider a parameter $\beta$, where $0<\beta<1$ (not-necessarily constant). The following statements are equivalent:

\begin{enumerate}
    \item[(i)] There is a $\beta$-approximation algorithm for \textbf{STO}.\label{beta-STO}
    
    \item[(ii)] There is a $\beta$-approximation algorithm for \textbf{NW-DRBP}.\label{beta-NW-DRBP}
\end{enumerate}
\end{lemma}

\begin{proof}
To prove that (i) implies (ii), we proceed as follows. Let $J=\langle D'= (V', A'), p', c', r', B' \rangle$ be an instance of \textbf{NW-DRBP}.
Let $I=\langle D= (V, A), p, c, r, B \rangle$ be an instance of \textbf{STO} obtained from $J$ as follows. We set $V=V'$, $r=r'$, $A=A'\setminus \{(v, r')| (v, r') \in A'\}$, $B=B'-c(r')$ and for any subset $S \subseteq V$, $p(S)=p'(S)$. For any $e=(i,j) \in A$ in $I$, we set $c(e)=c'(j)$. Consider a solution $T$ to \textbf{STO} on $I$. Now we obtain a solution $T'=(V'(T'), A'(T'))$ to \textbf{NW-DRBP} from $T=(V(T), E(T))$ as follows. We set $V'(T')=V(T)$ and $A'(T')=A(T)$. We conclude the first direction by noticing that $c'(T')=\sum_{v \in V(T')} c'(v)=\sum_{e=(u,v) \in A(T)}c(e)$ and $p'(T')=p(T)$.

Now we show that (ii) implies (i). %, we give a polynomial-time reduction from \textbf{RDTO} to \textbf{OWMaxP} as follows. 
Let $I=\langle D= (V, A), p, c, r, B \rangle$ be an instance of \textbf{STO}. Let $J=\langle D'= (V', A'), p', c', r', B' \rangle$ be an instance of \textbf{NW-DRBP} obtained from $I$ as follows.
\begin{itemize}
    \item $V' = V \cup V_{A}$ with $V_{A} = \{v_e : e \in A\}$. 
    \item $A' = \{(i, v_e), (v_e, j):  e=(i,j)\in A\}$. 
\end{itemize}


We set $r'=r$ and $B'=B$. Each subset $S \subseteq V'$ is assigned with prize $p'(S)=p(S\setminus V_A)$. Note that $p(\emptyset)=0$. Each vertex $v \in V' \cap V$ (resp. $v_e \in V' \cap V_{A}$) is assigned with a cost $c'(v)=0$ (resp. $c'(v_e)=c(e)$). Consider a solution $T'=(V'(T'), A'(T'))$ to \textbf{NW-RDBP} on $J$. Note that in $T'$ if there is a leaf $l \in V_A$, the next node $v \in e=(l, v)$ can be added to the solution $T'$ as cost $c'(v)=0$ and prize $p'(V'(T') \cup \{l\})\ge p'(V'(T'))$ (by the monotonicity of $p'$). From $T'$, we obtain $T=(V(T), A(T))$ as follows. We set $V(T) = V'(T') \cap V$ and $A(T) = \{ e=(i,j):  (i, v_e), (v_e, j)\in A'(T')\}$. For any $e \in A(T)$, we set $c(e)=c'(v_e)$. The proof follows from $c(T)=\sum_{e=(u,v) \in A(T)}c(e)=\sum_{v_e \in V'(T') \cap V_A} c'(v_e)=c'(T')$ and $p(T)=p'(T')$.
\end{proof}


By Theorem~\ref{thGhugeEW-RDBPQuasiAlgorithm} and Lemma~\ref{thGhugeNagarajanNW-DRBP}, we have the following theorem.

\begin{theorem}\label{thGhugeNagarajanNW-DRBP}
There is an $O(\frac{\log k}{\log \log k})$-approximation
algorithm for \textbf{NW-DRBP} that runs in
$(n \log B)^{O(\log^{1+\epsilon} k)}$ time for any constant $\epsilon > 0$, where $k \le n=|V|$ is the number of vertices in an optimal solution.
\end{theorem}




==> contribution/application.tex <==
\section{Variants of \textbf{NW-DRBP}}

In this section, we consider some important variants of \textbf{NW-DRBP} and show that our technique for \textbf{NW-DRBP} can be utilized to obtain some polynomial-time approximation algorithms for these variants.

\input{contribution/Application/STO}
\input{contribution/Application/MCSB}
\input{contribution/Application/NW-RBP}
\input{contribution/Application/NW-RQP}
\input{contribution/Application/Connected-Maximum-Set-Coverage}
\input{contribution/Application/Budgeted-Sensor-Cover}
\input{contribution/Application/Budgeted-Connected-Dominating-Set}

==> contribution/uto.tex <==
\section{Complexity Results for \textbf{EW-RBP}}

As a warm up, we first show that \textbf{EW-RBP} is NP-hard even when given graphs are \textit{stars}. A star (or star graph) $S^*=(V, E)$ is a tree consisting of a vertex $r \in V$, called the root of $S^*$, attached to degree-1 vertices $v \in V\setminus \{r\}$, called the leaves of $S^*$, i.e., $E=\{\{r, v\}:v \in V \setminus\{r\}\}$. In other words, a star graph is a tree with only one vertex of degree more than one

\begin{theorem}\label{thUTOStar}
\textbf{EW-RBP} is NP-hard even on star graphs.
\end{theorem}

\begin{proof}
To prove the theorem, we give a reduction from the $0-1$ knapsack problem. Recall that in the $0-1$ knapsack problem, we are given a set $O=\{o_1, \dots, o_n\}$ of objects, a knapsack capacity $KC \in \mathbb{Z}^+$, and each object $o_i$ is assigned with a size $s(o_i) \in \mathbb{Z}^+$ and a weight $w(o_i) \in \mathbb{Z}^+$. The task is to find a subset $O' \subseteq $ of objects whose total size is bounded by $KC$, i.e., $s(O')=\sum_{o \in O'}s(o) \le KC$, and the total weight $s(O')=\sum_{o \in O'}w(o)$ is maximized. 

Given an instance $I=(O, KC)$ of the knapsack problem, an instance $I'$ of \textbf{EW-RBP} is obtained as follows. We create a star $S^*=(V,E)$ such that $V=\{v_i: o_i \in O\} \cup \{r^*\}$ and $E=\{\{r^*,v_i\}: o_i \in O\}$. Each vertex $v_i \in V\setminus \{r^*\}$ is assigned with a prize $p(v_i)=w(o_i)$, and $p(r^*)=0$. Each edge $\{r^*,v_i\}$ is associated with a cost $c(\{r^*,v_i\})=s(o_i)$. Let $B=KC$. Obviously, from any solution to $I$, we can create a solution to \textbf{EW-RBP} in polynomial time. The reverse direction is also straight forward.
\end{proof}

This hardness result motivated us to provide some positive results for \textbf{EW-RBP} when the input graphs are trees. In particular, we are able to modify the results given for the Knapsack problem~\cite{vazirani2013approximation} to provide some desired results for our problem on trees. \HG{I think it works but you have to be careful that weights can be negative so for instance taking the full tree if possible may not be optimal.}

\begin{theorem}\label{thUTOPseudo-Polynomial}
There is a pseudo-polynomial time algorithm for \textbf{EW-RBP} when the input graph $G=(V,E)$ is a tree which outputs a tree $T^*$ in time $O(n^2p_{max})$, where $p_{max}=max_{v \in V} p(v)$ and $n=|V|$.
\end{theorem}


\begin{proof}

Let $T=G$ be the given tree. If $\sum_{e \in E(T)} c(e) \le B$, we are done \HG{Can't the weights be negative no?}. Suppose it is not the case. Then we proceed as follows. Let $V(T)=\{1,2,\dots, n\}$ be the set of vertices in $T$ and $n=r^*$. We run a depth-first search of $T$ starting from $r^*$. Let $\pi_d$ be the ordering of vertices in $T$ such that vertices are sorted in decreasing order of their discovering times in the depth first search. 
As $n$ is first visited in the depth first search, it is the last voter in the ordering $\pi_d$. We define a table $F$ where $F[i,p]$ is the subtree with composed of a set $S \subseteq \{1,2,\dots, i\}$ with prize exactly $p$ and whose cost is minimized, where $i$ ranges from $0$ to $n-1$ and $p$ ranges from $1$ to $np_{max}$ \HG{Once again the weights can be negative, why $n-1$ and not $n$ ?}. Let $T(j) \subseteq T$ be the subtree rooted in a vertex $j$ and $t_j=|T(j)|$. Note that a subtree rooted at a vertex $j$ consists of all vertices whose path to the root of $T$ passes through $j$. The entries of this table will be filled as follows. For $i=0$ and $p \in \{1, \dots, np_{max}\}$ we have $F[0,p]=0$. For any $i$ and $p < p(i)$, we have $F[i,p]=F[i-t_i,p]$. When $p(i) \le p$, we define $F[i,p]=\min \{F[i-1, p-p(i)]+c_i, F[i-t_i, p]\}$. The first summand corresponds to the case that $i$ will be in the solution and there will be a path from $r^*$ to $i$. The second summand indicates that $i$ will not be in the solution, so $i$ and of course the subtree $T(i)$ will be removed from further consideration. After filling the table entries, we can determine which entry of the table contains the optimal weight to \textbf{EW-RBP} whose cost is less than or equal to $B$ as follows: $OPT=\max\{p| F[n-1, p] \le B\}$. Now comparing the first summand and the second summand will enable us to find out whether $i$ (and possibly its subtree) is in the final solution. Thus it takes $O(n^2p_{max})$ time to find an optimal solution.
%We define a table $F$ where $F[i,b]$ is the subtree with maximum weight composed of a set $S \subseteq \{1,2,\dots, i\}$ with cost at most $b$, where $i$ ranges from $0$ to $n-1$ and $b$ ranges from $1$ to $B$. Let $T(j) \subseteq T$ be the subtree rooted in a vertex $j$ and $t_j=|T(j)|$. Note that a subtree rooted at a vertex $j$ consists of all vertices whose path to the root of $T$ passes through $j$. The entries of this table will be filled as follows. Let $p_i$ be the parent of $i$ in $T$. For $i=0$, we have $F[0,b]=0$. For any $i$ and $b < c(\{i, p_i\})$, we have $F[i,b]=F[i-t_i,b]$. When $b \ge c(\{i, p_i\})$, we define $F[i,b]=\max \{F[i-1, b-c(\{p_i,i\})]+w_i, F[i-t_i, b]\}$. The first summand corresponds to the case that $i$ will be in the solution and there will be a path from $r^*$ to $i$ (directly or indirectly). The second summand indicates that $i$ will be not be in the solution, so $i$ and the subtree $T(i)$ will be removed from further consideration. After filling the table entries, comparing the first summand and the second summand will enable us to find out $i$ (and possibly its subtree) is in the final solution. Thus it takes $O(nB)$ time to find an optimal solution.
\end{proof}

We can utilize the FPTAS given for the Knapsack problem to present an FPTAS for \textbf{EW-RBP} on trees. 
\begin{theorem}
    There exists an FPTAS for \textbf{EW-RBP} on trees that runs in $O(n^2 \left \lfloor{\frac{n}{\epsilon}}\right \rfloor )$, where $n$ is the number of vertices and $\epsilon >0$.
\end{theorem}

\begin{proof}
%We first may run an alternative dynamic programming for \textbf{EW-RBP}, which finds an optimal solution, as follows. Note that $n w_{max}$ is the maximum weight an optimal solution $T^*$ can have. As Theorem~\ref{thUTOPseudo-Polynomial}, we first sort vertices in decreasing order of their discovering times in the depth first search. We define a table $F$ where $F[i,w]$ is the subtree with maximum weight composed of a set $S \subseteq \{1,2,\dots, i\}$ with weight exactly $w$ and whose cost is minimized, where $i$ ranges from $0$ to $n-1$ and $w$ ranges from $1$ to $nw_{max}$. Let $T(j) \subseteq T$ be the subtree rooted in a vertex $j$ and $t_j=|T(j)|$. Note that a subtree rooted at a vertex $j$ consists of all vertices whose path to the root of $T$ passes through $j$. The entries of this table will be filled as follows. For $i=0$ and $w \in \{1, \dots, nw_{max}\}$ we have $F[0,w]=0$. For any $i$ and $w < \omega(i)$, we have $F[i,w]=F[i-t_i,w]$. When $\omega(i) \le w$, we define $F[i,w]=\min \{F[i-1, w-\omega(i)]+c_i, F[i-t_i, w]\}$. The first summand corresponds to the case that $i$ will be in the solution and there will be a path from $r^*$ to $i$ (directly or indirectly). The second summand indicates that $i$ will be not be in the solution, so $i$ and the subtree $T(i)$ will be removed from further consideration. After filling the table entries, comparing the first summand and the second summand will enable us to find out $i$ (and possibly its subtree) is in the final solution. Thus it takes $O(n^2w_{max})$ time to find an optimal solution.

Let $T$ be the given tree. Let $P_T(i,j)$ be the path from vertex $i$ to $j$ in $T$ and $c(P_T(i,j))=\sum_{e \in P_T(i,j)} c(e)$. Let $V_{reach} $ be the set of vertices $v$ in $T$ such that $c(P_T(r^*,v)) \le B$. Given $\epsilon >0$ and let $K=\frac{\epsilon p_{max}}{n}$, where $p_{max}=max_{v \in V_{reach}} p(v)$ \HG{Rephrase sentence}. We can set new prize for each vertex $v \in V$ as $p'(v)=\left \lfloor{\frac{p(v)}{K}}\right \rfloor$. Now we can run the given dynamic-programming algorithm in Theorem~\ref{thUTOPseudo-Polynomial} for new weights. Let $T'$ be an optimal solution for \textbf{EW-RBP} on the new instance (i.e., the instance obtained from updating weights). Let $T^*$ be an optimal tree before updating the weights. Because of rounding down, $K.p'(v) \le p(v)$ for any $v \in V(T)$ \HG{Why ?}. So, we have 

$$p(T^*)-K.p'(T^*) \le nK.$$

The dynamic-programming algorithm must return a set at least as good as $T^*$ under the new weights. Let $OPT=p(T^*)$. Therefore,

\begin{align*}
    p(T') \ge K.p'(T^*) \ge p(T^*)-nK=OPT- \epsilon p_{max} \ge (1-\epsilon) OPT,
\end{align*}
where the last inequality holds as $OPT \ge p_{max}$ \HG{This may not be true if weights can be negative but this can be solved}.
\end{proof}
%%%%%%%%%%%%%%%%
%We next show that \textbf{EW-RBP} cannot be approximated in polynomial time with an approximation ratio better than $1-1/e$ if $P\neq NP$. The approximation preserving reduction used is from the maximum coverage problem.

We next show that \textbf{EW-RBP} is NP-hard even when all the costs are the same and equal to $1$ and all the weights are either $0$ or $1$.


\begin{theorem}\label{thEW-RBPMaximumDeg3}
	\textbf{EW-RBP} is NP-hard, even when in a given graph $G=(V,E)$, $\forall i \in V$, $p_i \in \{0,1\}$ and $\forall e \in E$, $c(e)=1$.
\end{theorem}


%We need the following observations to prove Theorem~\ref{thEW-RBPMaximumDeg3}. We give a reduction from an instance $I$ of the maximum coverage problem to an instance $ J $ of \textbf{EW-RBP}. Recall that in the maximum coverage problem, we are given a universe $ U = \{x_1,\ldots, x_N\}$ of $N$ elements, a collection $ S=\left\lbrace S_1, S_2, ..., S_M \right\rbrace $ of subsets of $ U $, and an integer $k$. We wish to find a subset $S' \subseteq S$ of sets such that $|S'| \le k$ and the number of covered elements $|\cup_{S_i \in S'}S_{i}|$ is maximized.% This problem is known to be hard to approximate better than $1 - 1/e$~\cite{feige1998threshold}. 

We need the following observations to prove Theorem~\ref{thEW-RBPMaximumDeg3}. We give a reduction from an instance $I$ of the minimum vertex cover problem to an instance $ J $ of \textbf{EW-RBP}. Recall that in the decision version of the minimum problem, we are given an undirected graph $G'=(V',E')$, and an integer $k$. We wish to determine whether there exists at most $k$ vertices in $V'$ that covers all the edges in $E'$.



\paragraph{The reduction.} 
    From an instance $I = (G'=(V', E'), k)$ of the minimum vertex problem, we create an instance $J=(G=(V,E), p,c,r,B)$ of \textbf{EW-RBP} with three layers of vertices as follows:
         
         \begin{enumerate}
             \item In the top layer, we have the root $r$ with prize $p_r=0$.
             
             %\item In the next layer, one set vertex $ v_{S_j} $ is created for each set $ S_j \in S $, associated with prize $p_{v_{S_j}}=0$ and connected to vertex $r$ via unit cost edge, i.e., $c(\{v_{S_j}, r\})=1$. Let $V_S$ be the set of all set vertices and $E_S$ be the set of all edges between $V_S$ and $r$, $E_S=V_S \times \{r\}$.
             \item In the next layer, one element vertex $v_i$ is created for each vertex $ i\in V' $, associated with prize $p_i=0$ and connected to vertex $r$ via unit cost edge, i.e., $c(\{v_i, r\})=1$. Let $V_S$ be the set of all element vertices and $E_S$ be the set of all edges between $V_S$ and $r$, $E_S=V_S \times \{r\}$.
             
             %\item The last layer contains an element vertex $v_{i}$ for each element $x_i \in U$, associated with prize $p_{v_{i}}=1$ and connected to a set vertex $v_{S_j}$ if $x_i \in S_j$ with cost $c(\{v_i, v_{S_j}\})=1$. Let $V_U$ be the set of all element vertices and $E_U$ be the set of all edges between $V_U$ and $V_S$, i.e., $\{v_i, v_{S_j}\} \in E_U$ if $x_i \in S_j$.
             
             \item The last layer contains an edge vertex $v_e$ for each edge $e \in E'$, associated with prize $p_{v_e}=1$ and connected to a vertex $v_i$ if $v_i \in e$ with cost $c(\{v_e, v_i\})=1$. Let $V_U$ be the set of all edge vertices and $E_U$ be the set of all edges between $V_U$ and $V_S$, i.e., $\{v_e, v_i\} \in E_U$ if $v_i \in v_e$.
         \end{enumerate}
         
We set $B=|E'|+k$. Note that $V=V_S \cup V_U \cup \{r\}$ and $E=E_S \cup E_U$. Let $\mathcal{T}$ be the set of trees of $G=(V,E)$ obtained from our reduction such that for any tree $T=(V_T, E_T) \in \mathcal{T}$, $r \in V_T$, where $V_T \subseteq V$ and $E_T \subseteq E$. For any pair of vertices $v, v' \in V_T$, let $P_T(v, v')$ be the path from $v$ to $v'$ in $T$ and let $c(P_T(v,v'))=\sum_{e \in P_T(v,v')}c(e)$. Obviously, in any tree $T \in \mathcal{T}$, each vertex $v_e \in V_T \cap V_U$ is reachable from $r$ by cost at least $2$ as from $r$ we need to pass at least one element vertex to reach $v_e$. Note that in any tree $T \in \mathcal{T}'$, $\forall v \in V_T \cap V_U$, $c(P(v,r))=2$ and $\forall v \in V_T \cap V_S$, $c(P(v,r))=1$. Let $\mathcal{T}' \subseteq \mathcal{T}$ be the set of all trees in which for any $T=(V_T, E_T) \in \mathcal{T}'$, the path between any vertex $v \in V_T$ and $r$ costs at most $2$, i.e., $\forall v \in V_T$, $c(P_T(v_e,r)) \le 2$. Let $\mathcal{T}'' = \mathcal{T}\setminus \mathcal{T}'$, i.e., in each tree $T''=(V_{T''}, E_{T''}) \in \mathcal{T}''$, for any $v \in V_{T''}$, $c(P_{T''}(v,r)) \ge 2$ and there exists at least one vertex $v' \in V_{T''}$ with $c(P_{T''}(v',r)) > 2$.
         
Now we would like to show that for any tree $T'' \in \mathcal{T}''$, one can obtain another tree $T'$ on the same vertices with the same cost in polynomial time such that $T' \in \mathcal{T}'$.
         
\begin{obs}\label{obsEW-RBPsameCost}
  For any tree $T''=(V_{T''}, E_{T''}) \in \mathcal{T}''$, one can obtain another tree $T'=(V_{T'}, E_{T'})\in \mathcal{T}$ in polynomial time such that $V_{T''}=V_{T'}$ and $c(T')= c(T'')$.
\end{obs}

\begin{proof}

 Consider an edge vertex $v_{e''} \in V_{T''} \cap V_U$ with $c(P_{T''}(v_{e''},r)) > 2$. We proceed as follows (we can have the same process for an element vertex $v'' \in V_{T''} \cap V_U$). Consider the path from $v_{e''}$ to $r$ in $T''$, $P_{T''}(v_{e''},r)=\{(v_{e''}, v_1), (v_1, v_2), \dots, (v_{z-1}, v_z), (v_{z},r)\}$. This implies that $z \ge 3$ as the path from $v_{e''}$ to $r$ contains at least two element vertices and one edge vertex except $v_{e''}$ itself. Of course $v_1$ is a element vertex as $c(P_{T''}(v_{e''},r)) > 2$ and walking from one edge vertex to another edge vertex requires us to pass through at least one element vertex. By the same argument we see that $v_2$ is an edge vertex. Hence, from $T''$ we can obtain another tree $T_1=(V_{T_1}, E_{T_1})$ such that $V_{T_1}=V_{T''}$, $E_{T_1}=E_{T''} \cup \{v_1, r\} \setminus \{v_1,v_2\}$ (i.e., replacing edge $\{v_1,v_2\}$ by edge $\{v_1, r\}$) and $c(T)=c(T'')$ (as for any $e \in E$, $c(e)=1$). This implies that $c(P_T(v_{e''},r))=2$. We can apply the same process for any element vertex $v'' \in V_{T''} \cap V_S$ if $c(P_T(v'',r)) \ge 2$. Now if for any vertex $v \in V_{T_1}$, $c(P_{T_1}(v,r)) \le 2$ then we are done. Otherwise, we repeat this process on $T_1$ until we obtain a tree $T_l$ in which any vertex $v \in V_{T_l}$ is reachable from $r$ by cost at most $2$, i.e., $T'=T_l \in \mathcal{T}'$. This can be done in polynomial time as each tree contains at most $|V'|+|E'|$ vertices, which concludes the proof.

\end{proof}

We are now ready to prove Theorem~\ref{thEW-RBPMaximumDeg3}.

\begin{proof}[Proof of Theorem~\ref{thEW-RBPMaximumDeg3}]
Let $I = (G'=(V', E'),k)$ be an instance of the minimum vertex cover problem, and $J=(G=(V,E), p,c,r,B)$ be the instance of \textbf{EW-RBP} resulting from our reduction. By Observation~\ref{obsEW-RBPsameCost}, we suppose that any solution $T$ to the instance $J$ is in the collection $\mathcal{T}'$ defined above. Recall that $r \in V_T$ and for any $v \in V_T \setminus \{r\}$, $c(P_T(r,v)) \le 2$. It is straight forward that there exists a solution $V''$ to $I$ with size $|V''| \le k$ that covers all the edges $E'$ if and only if there exists a solution (tree) $T \in \mathcal{T}'$ to $J$ with cost $ |E'| < c(T) \le |E'|+k$ and prize $p(T)=|E'|$.

%Now let $OPT=n$ be the optimum value of the maximum coverage instance and $S^*$ be an optimal solution. We obtain a tree $T^*$ to $J$ as follows. For any set $S_i \in S^*$, $v_{S_i}$ is connected to $r$ in $T$, i.e., $\{v_{S_i}, r\} \in E_{T^*}$. Any element vertex $v_x$ is connected to set vertex $v_{S_i}$ in $T$ if $x$ is covered by $S_i$ in solution $S^*$ (the choice of $S_i$ can be made arbitrarily if several sets cover $x$ in $S^*$). Hence, $p(T^*)=n$
\end{proof}


\begin{corollary}
\textbf{EW-RBP} is NP-hard, even when in a given graph $G=(V,E)$, $\forall i \in V$, $p_i \in \{0,1\}$, $\forall e \in E$, $c(e) \in \{0, 1\}$ and the maximum degree of a vertex is at most $3$.      
\end{corollary}

\begin{proof}[Sketch of proof]
We have almost the same reduction as that of Theorem~\ref{thEW-RBPMaximumDeg3}, there is only an additional path for each element vertex and one path between element vertices and vertex $r$. In particular, let $N_u$ be the set of edge vertices connected to the element vertex $u$ in the instance $J$ of \textbf{EW-RBP} resulting from our reduction in Theorem~\ref{thEW-RBPMaximumDeg3}. In our new instance $J'$, we have one additional path $P^u$ for each element vertex $u$ containing $|N_u|$ vertices, i.e., each vertex $v'_e \in P^u$ corresponds to an edge vertex $v_e$ entering $u$ in $J$. Now in $J'$, there is an edge connecting $v_e$ to $v'_e$ with unit cost. Each path $P^u$ costs zero, i.e., $c(P^u)=\sum_{v'_e \in P^u}c_{v'_e}=0$. Also, there is an edge connecting the head of each path $P^u$ to the element vertex $u$ with cost zero. Last, there is a path $P^r$ containing $|V_S|$ vertices, i.e., each vertex $u' \in P^r$ corresponds to an element vertex $u \in V_S$. Each element vertex $u$ connected to its corresponding vertex $u' \in P^r$ with cost $1$. $P^r$ costs zero, i.e., $\sum_{e \in P^r} c(e)=0$. Furthermore, there is an edge connecting the head of $P^r$ to $r$ with cost zero. This concludes the proof.
\end{proof}

However, there is a polynomial time algorithm for \textbf{EW-RBP} when the maximum degree of a vertex is at most $2$.

\begin{theorem}\label{thEW-RBPMaximumDeg2}
There is a polynomial time algorithm for \textbf{EW-RBP} when in the input graph $G=(V,E)$ the maximum degree of a vertex is at most $2$ which outputs a tree $T^*$ in time $O(n^4)$, where $n=|V|$.
\end{theorem}

\begin{proof}
Let $V_{reach}$ be the set of vertices that are reachable from $r$ in G. To prove the theorem, we distinguish between two cases.


\begin{enumerate}
    \item  Each vertex $v$ in $V_{reach}$ has degree exactly $2$. This implies that the graph $G[V_{reach}]$ induced by set of vertices $V_{reach}$ is a cycle. In this case, we proceed as follows: Let $C=(V_C, E_C)$ be the cycle in $G$ such that $r \in V_C$. Let $T_e=(V_{T_e}, E_{T_e})$ be the resulting tree after removing an edge $e$ from $E_{C}$, i.e., $V_{T_e}=V_C$ and $E_{T_e}=E_C\setminus \{e\}$. The number of subtrees of $T_e$ rooted at $r$ is at most $O(n^3)$. Then we select a feasible subtree $T^*_e$ of $T_e$ (i.e., $c(T_e) \le B$) with the maximum prize. We then output the tree $T^*_{e^*}$ where $T^*_{e^*}=\max_{p(T_e)} T^*_e$. This takes $O(n^4)$ times as $|E_C| \le n$.
    
    \item There are some vertices in $V_{reach}$ with degree less than $2$. This means that $r$ is on a path and it has at most $O(n^3)$ subtrees rooted at $r$. Thus we select a feasible subtree $T^*_e$ of this path with the maximum prize. This takes $O(n^3)$ times.
    
\end{enumerate}

This concludes the proof.
\end{proof}


%%%%%%%%%%%%%%%
We next aim to provide a pseudo-polynomial algorithm on a tree decomposition $\mathcal{T}=(T, \{X_t\}_{t \in V(T)})$ of width $k$ of undirected graph $G$ that outputs an optimal solution $T^*$ to \textbf{EW-RBP}. 

\begin{theorem}\label{thUTOTreeDecomposition}
Given a graph $G=(V,E)$ with tree decomposition $\mathcal{T}$ of width $k$. There exists a pseudo-polynomial algorithm that gives an optimal solution $T^*$ to \textbf{EW-RBP} in time $n.B.k^{O(k)}$, where $n=|V|$ and $B$ is the budget.
\end{theorem}

To do so, we follow some of the ideas have been used by Cygan et al.~\cite{cygan2015parameterized} for the STEINER TREE problem. In this approach, we will use a refined variant of nice tree decomposition, where the following conditions are satisfied:

\begin{itemize}
    \item $X_r=\emptyset$ and $X_l=\emptyset$ for every leaf $l \in T$, i.e., all the leaves as well as the root contain empty bags.
    \item Every non-leaf node of $T$ is one of the following four types:
    
    \begin{itemize}
        \item \textbf{Introduce node:} a node $t$ with exactly one child $t'$ such that $X_t = X_{t'} \cup \{v\}$ for some vertex $v \notin X_{t'}$; we say that $v$ is introduced at $t$.
        \item \textbf{Forget node:} a node $t$ with exactly one child $t'$ such that $X_t = X_{t'} \setminus \{u\}$ for some vertex $u \in X_{t'}$; we say that $u$ is forgotten at $t$.
        \item \textbf{Join node:} a node $t$ with two children $t_1, t_2$ such that $X_t = X_{t_1} = X_{t_2}$.
        \item \textbf{Introduce edge node:} a node $t$, labeled with an edge $uv \in E(G)$ such that $u, v \in X_t$, and with exactly one child $t'$ such that $X_t = X_{t'}$. We say that edge $uv$ is introduced at $t$.
    \end{itemize}
    
\end{itemize}

Note that in this extended version of a nice tree decomposition, every edge of $E(G)$ is introduced exactly once in the whole decomposition. Furthermore, leaf nodes, forget nodes and join nodes are defined just as the ones in the standard version of nice tree decomposition. To transform a standard nice tree decomposition to this variant, we proceed as follows. Consider an edge $\{u ,v\} \in E(G)$ and for any $v \in V(G)$, let $t(v)$ be the highest node in $T$ such that $v \in X_{t(v)}$. Without loss of generality assume that $t(v)$ is an ancestor of $t(u)$. To obtain this variant of nice tree decomposition, we insert the introduce edge bag that introduces $uv$ between $t(u)$ and its parent (which forgets $u$). The obtained tree decomposition has
$O(kn)$ nodes, since a graph of treewidth at most $k$ has at most $kn$ edges. We will denote this variant of nice tree decomposition by $\mathcal{T}=(T, \{X_t\}_{t \in V(T)})$. One last piece of notation: let $G_t$ be a subgraph of $G$ defined as follows: $G_t=(V_t, E_t)$, where $V_t$ is the union of all the bags present in the subtree of $T$ rooted at $t$ and $E_t$ is the set of all edges introduced in the subtree rooted at $t$. Now we are ready to prove Theorem~\ref{thUTOTreeDecomposition}

\begin{proof}[Theorem~\ref{thUTOTreeDecomposition}]
Given a graph $G$ and its nice tree decomposition $\mathcal{T}=(T, \{X_t\}_{t \in V(T)})$. To prove the theorem, we use a dynamic-programming algorithm part over $\mathcal{T}=(T, \{X_t\}_{t \in V(T)})$. For simplicity, we add $r^*$ to every bag of the tree decomposition $\mathcal{T}$. Consider an optimal solution $T^*$ to \textbf{EW-RBP}. Let $F_t$ be the part of $T^*$ contained in $G_t$. Obviously, $F_t$ is a forest and the intersection of $F_t$ and $X_t$ is not empty as $r^* \in X_t$ for any node $t$. Indeed, the main idea here is to find the intersection of $F_t$ and $X_t$ for any node $t \in T$. So, for any node $t$, the main task is to guess a partition $\mathcal{P}=\{P_1, \dots, P_q\}$ of $X_t$ such that each block $P_i \in \mathcal{P}$ is a part of a unique component of the forest $F_t$ in $G_t$. Now for a bag $X_t$, a set $X \subseteq X_t$ and a partition $\mathcal{P}=\{P_1, \dots, P_q\}$ of $X$, the value of $\mathcal{F}[t,X,\mathcal{P},B']$ is the maximum prize of vertices of a forest $F_t$ in $G_t$ respecting the budget $B'$ such that: i) $F_t$ has exactly $q$ connected components that can be ordered as $C_1, \dots, C_q$ so that $P_s=V(C_s) \cap X_t$ for each $s \in \{1, \dots, q\}$, i.e., $\mathcal{P}=\{P_1, \dots, P_q\}$ corresponding to connected components of $F_t$. ii) $X_t \cap V(F_t)=X$, i.e., the vertices of $X_t \setminus X$ are untouched by $F_t$.

Note that the optimal solution to \textbf{EW-RBP} is exactly $\mathcal{F}[r,\{r^*\},\{\{r^*\}\},B]$, where $r$ is the root of a tree decomposition $\mathcal{T}$ and $B$ is the budget. For $B=0$, we set $\mathcal{F}[t,X,\mathcal{P},0]=0$. We now provide a recursive formulas to compute the values of $\mathcal{F}$.

\paragraph{Leaf node.} If $t$ is a leaf node, $X_t=\{r^*\}$. We have $\mathcal{F}[t,\emptyset,\emptyset,B']=-\infty$ and $\mathcal{F}[t,\{r^*\},\{\{r^*\}\},B']=0$.

\paragraph{Introduce vertex node.} Let $t$ be an introduce vertex node with a child $t'$ such that $X_t=X_{t'} \cup \{v\}$ for some $v \notin X_{t'}$. If $v=r^*$ then for all $X \subseteq X_t$ not containing $v$, $\mathcal{F}[t,X,\mathcal{P},B']=-\infty$. $v$ is an isolated vertex in $G_t$ as $v$ has not introduced any edge in $G_t$. We call all partitions $\mathcal{P}$ of $X$ where $\{v\} \in \mathcal{P}$ valid as $v$ is an isolated vertex. If a partition $\mathcal{P}$ is not valid, we set $\mathcal{F}[t,X,\mathcal{P},B']=-\infty$. In other cases, we have 

\begin{align*}
\mathcal{F}[t,X,\mathcal{P},B'] \!=\! \left\{ \begin{array}{c c}
\mathcal{F}[t',X\setminus \{v\},\mathcal{P} \setminus\{\{v\}\},B'] & \text{ if } v \in X\\
\mathcal{F}[t',X,\mathcal{P},B'] & \text{ otherwise.}
\end{array} \right.
\end{align*}

\paragraph{Introduce edge node.} Let $t$ be an introduce edge node that introduces an edge $uv$, and let $t'$ be the child of $t$. If $u \notin X$ or $v \notin X$, edge $e=\{u,v\}$ would not be in $T^*$ as one of the endpoints of $e$ is not in $T^*$. Hence in this case $\mathcal{F}[t,X,\mathcal{P},B']=\mathcal{F}[t',X,\mathcal{P},B']$. The same happens if $u \in P_i$ and $v \in P_j$, where $P_i, P_j \in \mathcal{P}$ and $i \neq j$. Suppose that $u, v \in P_i$. In this case we have two options: either $e$ is picked or not. Let $\mathcal{P}'$ those partitions where $u$ and $v$ are in separate blocks (so that adding the $\{u, v\}$ does not create a cycle) and after merging the blocks containing $u$ and $v$ we obtain the partition $\mathcal{P}$. Then we have the following.

\begin{align*}
\mathcal{F}[t,X,\mathcal{P},B'] \!=\! \left\{ \begin{array}{c c}
\mathcal{F}[t',X,\mathcal{P},B'] & \text{ if } v \notin X \text{ or } u \notin X\\
\mathcal{F}[t',X,\mathcal{P},B'] & \text{ if $u \in P_i$, $v \in P_j$ and $i \neq j$}\\
\max\{\max_{\mathcal{P}'}{\mathcal{F}[t',X,\mathcal{P}',B'-c(\{u,v\})]}, \mathcal{F}[t',X,\mathcal{P},B']\}& \text{otherwise.}
\end{array} \right.
\end{align*}

\paragraph{Forget node.} Let $t$ be a forget node and $t'$ be its child. Then $X_t=X_{t'} \setminus \{t\}$. $v$ belongs to $F_t$ or not. Let $\mathcal{P}'$ be a partition obtained from a partition $\mathcal{P}$ of $X$ by adding $v$ into one of the blocks $P_i \in \mathcal{P}$. Hence

$$\mathcal{F}[t,X,\mathcal{P},B'] =\max\{\max_{\mathcal{P}'}\{\mathcal{F}[t',X \cup \{v\},\mathcal{P}',B'] + \omega(v)\}, \mathcal{F}[t',X,\mathcal{P},B']\}.$$


\paragraph{Join node.} Suppose that $t$ is a join node with children $t_1$ and $t_2$. In this case, we need to merge two partial solutions: one is a solution to $G_{t_1}$ and the other one to $G_{t_2}$. Merging these two partial solutions may result in cycles. To avoid this, we need to try all pairs of partitions $\mathcal{P}_1$ and $\mathcal{P}_2$ of $X$ such that $\mathcal{P}$ is an acyclic merge of them. Therefore

$$\mathcal{F}[t,X,\mathcal{P},B']=\max_{\mathcal{P}_1, \mathcal{P}_2}\{\mathcal{F}[t',X,\mathcal{P}_1,B']+ \mathcal{F}[t',X,\mathcal{P}_2,B']\}.$$

This finishes our recursive formula. Now we move on to the running time of this dynamic-programming algorithm. Let $k$ be the tree-width of $\mathcal{T}$, i.e., $k$ is the size of bag with maximum size. At each bag, we need to expend $2^{k+1}.(k+1)^{k+1}=k^{O(k)}$ time since for any node $t$, there exists $2^{|X_t|}$ subsets $X \subseteq X_t$ and at most $|X|^{|X|}$ partitions. To compute the value for every state, we need to consider the pairs of states for some other nodes, i.e., each value is computed in time $O(k^{O(k)})$. As $\mathcal{T}$ has $O(kn)$ nodes, the total running time is $n.B.k^{O(k)}$.

\end{proof}


Next we would like to show that \textbf{NW-RBP} is a more general case of \textbf{EW-RBP}. Note that \textbf{NW-RBP} has been stated in the Related Work section~\ref{secRW}.

\begin{obs}\label{obsRBPandUTO}
\textbf{NW-RBP} is a more general case of \textbf{EW-RBP}.
\end{obs}

\begin{proof}
Consider an instance $I=\langle G'= (V', E'), w, c', r', B' \rangle$ of \textbf{EW-RBP}. We create an instance $I=\langle G= (V, E), p, c, r, B \rangle$ of \textbf{NW-RBP} as follows. We set $r=r'$ and $B=B'$. We create graph $G=(V, E)$ as follows. 

\begin{itemize}
    \item $V = V' \cup V_1$ with $V_1 = \{v_e : e \in E'\}$. 
    \item $E = \{\{i, v_e\}, \{v_e, j\}:  e=\{i,j\}\in A(T)\}$. 
\end{itemize}

Each vertex $v \in V \cap V'$ (resp. $v_e \in V \cap V_1$) is assigned with a prize $p(v)=w(v)$ (resp. $p(v_e)=0$) and a cost $c(v)=0$ (resp. $c(v_e)=c'(e)$). Now consider a solution $T=(V(T), E(T))$ to \textbf{NW-RBP} on $I$. We can obtain a solution $T'=(V(T'), E(T'))$ to \textbf{EW-RBP} on instance $I'$. We set $V(T')=V' \cap V(T)$. We have $e \in E(T')$ if $v_e \in E(T)$. For any $e \in V(T')$, we set $c'(e)=c(v_e)$ and any $v \in V(T')$, $w(v)=p(v)$. We conclude by noticing that there is no leaf $l \in T(V)$ with $l=v_e$ as, by construction, we have only two edges $e=\{i, v_e\}$ and $e'=\{l, u\}$ that contain $v_e$, and $c(v)=c(u)=0$.
\end{proof}
